Learning Computational Efficient Bots with Costly Features

Deep reinforcement learning (DRL) techniques have become increasingly used in various fields for decision-making processes. However, a challenge that often arises is the trade-off between both the computational efficiency of the decision-making process and the ability of the learned agent to solve a particular task. This is particularly critical in real-time settings such as video games where the agent needs to take relevant decisions at a very high frequency, with a very limited inference time. In this work, we propose a generic offline learning approach where the computation cost of the input features is taken into account. We derive the Budgeted Decision Transformer as an extension of the Decision Transformer that incorporates cost constraints to limit its cost at inference. As a result, the model can dynamically choose the best input features at each timestep. We demonstrate the effectiveness of our method on several tasks, including D4RL benchmarks and complex 3D environments similar to those found in video games, and show that it can achieve similar performance while using significantly fewer computational resources compared to classical approaches.

==> 6_experimental_details.tex <==
\newpage

\section{Experimental Details}
\label{section:exp_details}

The implementation of our algorithms and models is based on SaLinA \cite{bib_salina}, a python library built as an extension of the PyTorch one \cite{bib_pytorch} to efficiently develop sequential decision models. The source code is joined with the submission and will be open-sourced upon acceptance. 

\subsection{Environments}
\label{subsection:environments}

\subsubsection{D4RL}
\label{subsubsub:openai_gym}

In order to assess whether or not our algorithms are indeed able to train cost efficient agents, we study their performance on classical reinforcement learning tasks from the OpenAI \textbf{Gym} library \cite{bib_openai_gym}, namely HalfCheetah, Hopper and Walker2D which are illustrated in the Figure \ref{d4rlnv}. For each, the goal is to run as fast as possible and the farthest possible given a time limit. All three environments use the \textbf{MuJoCo} engine (\textbf{Mu}lti-\textbf{Jo}int dynamics with \textbf{Co}ntact), and the features available are the angle of the agent joints and their corresponding speed.

\begin{figure}[!ht]

    \centering
    \begin{minipage}[!ht]{0.30\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/HC.png}
        \subfloat{(A) HalfCheetah.}
        %\label{HC}
    \end{minipage}
    \hspace{0.02\linewidth}
    \begin{minipage}[!ht]{0.30\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/HOP.jpg}
        \subfloat{(B) Hopper.}
        %\label{W2D}
    \end{minipage}
    \hspace{0.02\linewidth}
    \begin{minipage}[!ht]{0.30\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/W2D.jpg}
        \subfloat{(C) Walker2D.}
        %\label{W2D}
    \end{minipage}
\caption{Visualization of the D4RL environments studied.}
\label{d4rlnv}
\end{figure}

Since we consider an Offline Reinforcement Learning approach, we leverage the benchmarked datasets of trajectories proposed by D4RL \cite{fu2020d4rl} so as to train our agents.

During evaluation, at each timestep the reward obtained is a scaled difference between the relative distance covered and a penalization term for an excessively wide action. To facilitate comparisons between the different tasks, D4RL provides the following normalization function given a score $S$, an expert score $S_{expert}$, and $S_{random}$ the score obtained by an agent with random actions:
\begin{equation}
    100\times\frac{S-S_{random}}{S_{expert}-S_{random}}
    \label{normalization_d4rl}
\end{equation}

\subsubsection{3D Navigation}
\label{subsubsection:smartnav}

The 3D Navigation environment is defined using the free and open-source game engine called Godot \cite{bib_godot_rl}. It is almost similar to the the environment used in \cite{roy2021direct} but has been reimplemented in Godot to rely on an open-source engine instead of Unity.

\begin{figure}[t!]
\label{figgdot}
    \centering
    \begin{minipage}[h!]{0.47\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/godot_close_up.png}
        \subfloat{(A) Close-up of to the agent.}
        %\label{HC}
    \end{minipage}
    \hspace{0.02\linewidth}
    \begin{minipage}[h!]{0.47\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/godot_snapshot.png}
        \subfloat{(B) View of a map.}
        %\label{W2D}
    \end{minipage}
\caption{Visualization of the Godot-based environments.}
\end{figure}

In this environment, an agent has to move toward a goal location in different maps. These maps are directly modeled after a [anomimity] AAA game. For this paper, we have chosen two maps with hard (open world environment) and easy (Arena environment) difficulties, defined based on obstacles and terrain. A positive reward is given to the agent whenever it gets closer to the goal location (the goal location varying at each episode) than it has been this episode, while avoiding lava and water (which kill the agent). 
The obstacles include water and lava on the path of the agent. The easy map is modeled with no obstacles, whereas the hard map is a larger and richer map in terms of obstacles and terrain. There are 1000 randomly chosen goal positions in each of the maps that are used at training time. At test time, we generate 256 new random starting and goal positions to evaluate the ability of the agent to handle unknown trajectories. The performance of the agent can be evaluated through a reward function that we have defined, or by its success rate. To generate the training dataset, we used the SAC algorithm abnd and saved the episodes generated by the learned agent at different performance levels. Note that, in the hard map, an expert policy trained using SAC has success\_fail around $95\%$, average episode returns $\sim 2.3$, and an average episode length of $\sim 50$ steps.

% \textcolor{red}{Describe the groups of raycasts here}

\subsection{Models}
\label{subsection:models}

We provide details about the architecture of the different models.


\paragraph*{MLP Architecture}

In the memory-less setting, we implement BC with 3 hidden layers of size 256 (see Table \ref{expe_details_bc}). RCBC is just an extension of this model where the reward-to-go corresponds to an additional feature, while IQL is using the same architecture. The details of the hyper-parameters are given in Tables \ref{expe_details_bc}



\paragraph{Budgeted Decision Transformers}

For the budgeted decision transformer, we rely on the same parametrization than the original Decision Transformer architecture -- see Table \ref{expedetailsdt}.


\begin{table}[h!]
    \footnotesize
    \centering
    \begin{tblr}{
        colspec = c c,
    }
        \hline
        \textbf{Hyperparameter} & \textbf{Value}\\
        \hline
        Number of layers & 3 \\
        Hidden size & 256 \\
        Layer activation function & ReLU \\
        Output activation function & TanH \\
        Batch size & 64 \\
        Dropout & $10^{-1}$ \\
        Learning rate & $10^{-4}$ \\
        Weight decay & $10^{-4}$ \\
        Gradient clipping & $2.0$ \\
        \hline
    \end{tblr}
    \caption{Hyperparameters of Behavioral Cloning (with MLP).}
\label{expe_details_bc}
\end{table}



\begin{table}[h!]
    \footnotesize
    \centering
    \begin{tblr}{
        colspec = c c,
    }
        \hline
        \textbf{Hyperparameter} & \textbf{Value}\\
        \hline
        Number of layers & 3 \\
        Number of attention heads & 1 \\
        Embedding dimension & 128 \\
        Layer activation function & ReLU \\
        Output activation function & TanH \\
        Context length & 20 \\
        Batch size & 64 \\
        Dropout & $10^{-1}$ \\
        Learning rate & $10^{-4}$ \\
        Weight decay & $10^{-4}$ \\
        Gradient clipping & $0.25$ \\
        \hline
    \end{tblr}
    \caption{Hyperparameters of Decision Transformer model.}
    \label{expedetailsdt}
\end{table}



==> 7_detailed_results.tex <==
\newpage

\section{Experimental Results Details}
\label{section:results_details}

We provide the complete results obtained on the different models in the different settings described in the main article. 

\subsection{Comparison with already published results On D4RL}

As a first set of experiments, we have validated that our implementations with $\gamma=0$ (aka n cost constraint) obtained the same performance as already published performance -- Table \ref{a1_baseline_rewards_d4rl}. Our implementations are on par with previously published results and the implementations are provided in the supplementary material. 

% \begin{figure}[h!]
% \label{baseline_d4rl_png}
%     \centering
%     \begin{minipage}[h!]{0.99\linewidth}
%         \centering
%         \includegraphics[width=1\linewidth]{images/baseline_d4rl.png}
%     \end{minipage}
% \caption{Average normalized cumulative rewards for cost-free models on OpenAI Gym environments.}

% \end{figure}

\subsection{Baselines for 3D Navigation}

We provide the baselines performances (without cost constraint) on the 3D navigation environments in Table \ref{a1_baseline_rewards_godot}

\subsection{Complete Results over D4RL Environments}

The complete results of the different models under cost constraints over the three D4RL environments, using the three available training datasets are provided in Table \ref{a1_budget_rewards_d4rl_expert_stochastic},\ref{a1_budget_rewards_d4rl_medium_expert_stochastic},\ref{a1_budget_rewards_d4rl_medium_stochastic}

\subsection{D4RL Environments with a varying cost window}

Instead of computing the cost at each timestep and constraining it, it is possible to extend the model to constrain the average cost of $N$ timesteps. It may allow the model to dispatch its budget over multiple timesteps, giving it more freedom degrees to acquire the relevant features. Table \ref{a1_budget_rewards_d4rl_cost_window} shows the performance over D4RL when changing the size of the cost window. Depending on the training dataset, increasing this size may increase the quality of the models, but the differences are not critical, justifying our focus on window sizes of size $N=1$ in the main paper.




% ====

\input{tables/baseline_d4rl.tex}
\input{tables/baseline_godot.tex}

\input{tables/question_1_d4rl_1.tex}
\input{tables/question_1_d4rl_2.tex}
\input{tables/question_1_d4rl_3.tex}

\input{tables/budget_godot}

% \input{tables/question_3_d4rl.tex}
\input{tables/question_2_d4rl.tex}

==> tables/baseline_d4rl.tex <==
\begin{table*}[!b]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|c|,
        row{1-2} = {pink},
        row{3-5} = {mygray},
        row{9-11} = {mygray},
        row{15-16} = {mydarkgray},
    }
        \hline
        \textbf{Dataset} & \textbf{Environment} & \textbf{DT} & \textbf{DT} & \textbf{DT} & \textbf{IQL} & \textbf{IQL} & \textbf{RCBC} & \textbf{RCBC} & \textbf{BC} \\
        & & \textbf{(RTG)} & \textbf{(No RTG)} & \textbf{(Original)} & & \textbf{(Original)} & \textbf{(RTG)} & \textbf{(No RTG)} & \\
        \hline
        & HalfCheetah & 92.4 $\pm$ 0.5 & 92.6 $\pm$ 0.4 & - & 91.4 $\pm$ 2.3 & - & 92.5 $\pm$ 0.2 & 92.7 $\pm$ 0.2 & 93.0 $\pm$ 0.2 \\
        Expert & Hopper & 110.4 $\pm$ 0.6 & 108.3 $\pm$ 4.9 & - & 98.3 $\pm$ 7.9 & - & 109.9 $\pm$ 0.9 & 109.8 $\pm$ 1.5 & 111.0 $\pm$ 0.4 \\
        & Walker2D & 108.3 $\pm$ 0.3 & 108.5 $\pm$ 0.4 & - & 112.2 $\pm$ 2.1 & - & 108.8 $\pm$ 0.3 & 108.8 $\pm$ 0.1 & 108.9 $\pm$ 0.2 \\
        \hline
        & HalfCheetah & 92.5 $\pm$ 0.4 & 73.7 $\pm$ 7.0 & 86.8 $\pm$ 1.3 & 85.0 $\pm$ 5.6 & 86.7 & 89.9 $\pm$ 0.4 & 75.4 $\pm$ 2.8 & 45.7 $\pm$ 1.3 \\
        Medium-Expert & Hopper & 108.2 $\pm$ 4.4 & 83.9 $\pm$ 37.2 & 107.6 $\pm$ 1.8 & 100.1 $\pm$ 11.5 & 91.5 & 107.6 $\pm$ 1.6 & 54.9 $\pm$ 1.2 & 61.9 $\pm$ 3.9 \\
        & Walker2D & 108.5 $\pm$ 0.4 & 107.1 $\pm$ 1.6 & 108.1 $\pm$ 0.2 & 108.6 $\pm$ 2.3 & 109.6 & 107.3 $\pm$ 1.7 & 106.2 $\pm$ 1.9 & 108.6 $\pm$ 0.4 \\
        \hline
        & HalfCheetah & 42.5 $\pm$ 0.2 & 42.6 $\pm$ 0.1 & 42.6 $\pm$ 0.1 & 47.3 $\pm$ 0.3 & 47.4 & 42.7 $\pm$ 0.2 & 42.5 $\pm$ 0.1 & 42.6 $\pm$ 0.2 \\
        Medium & Hopper & 64.3 $\pm$ 4.2 & 51.6 $\pm$ 4.8 & 67.6 $\pm$ 1.0 & 77.6 $\pm$ 5.8 & 66.3 & 66.1 $\pm$ 2.6 & 56.9 $\pm$ 1.6 & 54.8 $\pm$ 1.4 \\
        & Walker2D & 71.0 $\pm$ 3.1 & 68.9 $\pm$ 6.2 & 74.0 $\pm$ 1.4 & 76.5 $\pm$ 3.1 & 78.3 & 75.2 $\pm$ 1.2 & 73.1 $\pm$ 1.4 & 73.2 $\pm$ 0.9 \\
        \hline
        & HalfCheetah & 38.0 $\pm$ 1.1 & 34.1 $\pm$ 1.5 & 36.6 $\pm$ 0.8 & 44.2 $\pm$ 0.3 & 44.2 & 38.1 $\pm$ 0.5 & 32.6 $\pm$ 2.8 & 34.7 $\pm$ 2.2 \\
        Medium-Replay & Hopper & 83.1 $\pm$ 8.4 & 29.3 $\pm$ 7.4 & 82.7 $\pm$ 7.0 & 93.3 $\pm$ 5.8 & 94.7 & 75.4 $\pm$ 11.0 & 28.2 $\pm$ 3.8 & 30.2 $\pm$ 1.6 \\
        & Walker2D & 68.2 $\pm$ 2.7 & 31.6 $\pm$ 6.0 & 66.6 $\pm$ 3.0 & 77.9 $\pm$ 2.4 & 73.9 & 66.7 $\pm$ 3.6 & 23.0 $\pm$ 21.4 & 31.3 $\pm$ 14.3 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average (Without Expert)} & & 75.1 & 58.1 & 74.7 & 78.9 & 76.9 & 74.3 & 54.8 & 53.7 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average (With Expert)} & & 82.3 & 69.4 & - & 84.4 & - & 81.7 & 67.0 & 66.3 \\
        \hline
    \end{tblr}
    \caption{Average normalized cumulative rewards for query-free models on OpenAI Gym environments.\\
    These experiments allow us to validate the action component implementation of each model,
    as DT and IQL achieve
    close performances to the original papers,
    and to set the baseline for a quantitative study of our different budgeted models.}
\label{a1_baseline_rewards_d4rl}
\end{table*}

==> tables/baseline_godot.tex <==
\begin{table*}[!h]
    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|,
        row{1-2} = {pink},
        row{3-4} = {mygray},
        row{7-8} = {mygray},
        row{11-12} = {mydarkgray},
    }
        \hline
        \textbf{Dataset} & \textbf{Environment} & \textbf{DT} & \textbf{DT} & \textbf{RCBC} & \textbf{RCBC} & \textbf{BC} \\
        & & \textbf{(RTG)} & \textbf{(No RTG)} & \textbf{(RTG)} & \textbf{(No RTG)} & \\
        \hline
        Expert & EasyMap
        & R = 102.6 $\pm$ 0.6 & R = 102.1 $\pm$ 0.3 & R = 101.9 $\pm$ 0.4 & R = 101.9 $\pm$ 0.4 & R = 101.6 $\pm$ 0.4 \\
        & & S = 79.6 $\pm$ 0.7 & S = 78.9 $\pm$ 0.4 & S = 70.9 $\pm$ 0.8 & S = 72.6 $\pm$ 0.5 & S = 72.6 $\pm$ 0.5 \\
        \hline
        Expert & HardMap 
        & R = 82.7 $\pm$ 1.0 & R = 80.8 $\pm$ 2.3 & R = 76.2 $\pm$ 1.0 & R = 76.8 $\pm$ 1.1 & R = 77.6 $\pm$ 1.2 \\
        & & S = 79.6 $\pm$ 0.9 & S = 78.9 $\pm$ 2.9 & S = 70.9 $\pm$ 0.6 & S = 72.6 $\pm$ 1.6 & S = 72.6 $\pm$ 1.1 \\
        \hline
        Intermediate & EasyMap
        & R = 101.4 $\pm$ 0.7 & R = 101.2 $\pm$ 0.3 & R = 101.9 $\pm$ 0.7 & R = 100.9 $\pm$ 0.5 & R = 99.9 $\pm$ 1.0 \\
        & & S = 96.5 $\pm$ 0.8 & S = 96.3 $\pm$ 0.3 & S = 96.9 $\pm$ 0.9 & S = 95.9 $\pm$ 0.6 & S = 94.3 $\pm$ 1.1 \\
        \hline
        Intermediate & HardMap
        & R = 52.2 $\pm$ 1.7 & R = 50.9 $\pm$ 0.9 & R = 50.2 $\pm$ 1.3 & R = 48.7 $\pm$ 0.9 & R = 46.7 $\pm$ 1.4 \\
        & & S = 47.3 $\pm$ 1.9 & S = 45.6 $\pm$ 1.0 & S = 43.5 $\pm$ 1.8 & S = 41.6 $\pm$ 1.0 & S = 39.5 $\pm$ 0.9 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average Reward}
        & & R = 84.7 & R = 83.8 & R = 82.6 & R = 82.1 & R = 81.4 \\
        \SetCell[c=2]{c}{Average Success}
        & & S = 80.0 & S = 79.2 & S = 76.7 & S = 76.4 & S = 75.4 \\
        \hline
    \end{tblr}
    \caption{Average normalized cumulative rewards (R) and Averaged success rate (S) for cost-free models on the 3D navigation environment without cost constraint. These experiments set the baseline for a quantitative study of our budgeted models.}
\label{a1_baseline_rewards_godot}
\end{table*}

==> tables/budget_godot.tex <==

\begin{table*}[!h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-14} = {mygray},
        row{15} = {mydarkgray},
        row{28} = {mydarkgray},
        row{29-40} = {mygray},
        row{41} = {mydarkgray},
    }
        \hline
        \textbf{Environment} & \textbf{Type} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % Easy-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 102.6 $\pm$ 0.6
            & 100.0 $\%$ $\vert$\ R = 101.9 $\pm$ 0.4
            & 100.0 $\%$ $\vert$\ R = 101.6 $\pm$ 0.4 \\
        
        \hline
        
        & & & {\color{brown} 12.5 $\pm$ 0.2 $\%$} & {\color{brown} 23.3 $\pm$ 0.3 $\%$} & {\color{brown} 19.2 $\pm$ 0.0 $\%$}\\
        EasyMap & Expert & 50 $\%$
        & {\color{teal}R = 102.3 $\pm$ 0.3} & {\color{teal}R = 101.8 $\pm$ 0.9} & {\color{teal}R = 101.6 $\pm$ 0.2}\\
        & & & {\color{teal}S = 96.2 $\pm$ 0.5} & {\color{teal}S = 95.8 $\pm$ 1.2} & {\color{teal}S = 95.0 $\pm$ 0.0}\\
        
        \hline
        
        & & & {\color{brown} 9.7 $\pm$ 0.2 $\%$} & {\color{brown} 8.0 $\pm$ 0.4 $\%$} & {\color{brown} 7.3 $\pm$ 1.0 $\%$}\\
        EasyMap & Expert & 10 $\%$
        & {\color{teal}R = 102.3 $\pm$ 0.4} & {\color{teal}R = 102.3 $\pm$ 0.3} & {\color{teal}R = 101.0 $\pm$ 1.0}\\
        & & & {\color{teal}S = 96.4 $\pm$ 0.4} & {\color{teal}S = 96.0 $\pm$ 0.5} & {\color{teal}S = 94.8 $\pm$ 1.6}\\
        
        \hline
        
        & & & {\color{brown} 4.2 $\pm$ 0.1 $\%$} & {\color{brown} 0.7 $\pm$ 0.2 $\%$} & {\color{brown} 0.9 $\pm$ 0.1 $\%$}\\
        EasyMap & Expert & 1 $\%$
        & {\color{teal}R = 101.6 $\pm$ 0.5} & {\color{teal}R = 102.1 $\pm$ 1.1} & {\color{teal}R = 101.3 $\pm$ 0.2}\\
        & & & {\color{teal}S = 95.3 $\pm$ 1.2} & {\color{teal}S = 96.7 $\pm$ 2.4} & {\color{teal}S = 95.2 $\pm$ 0.7}\\
        
        \hline
        
        & & & {\color{brown} 3.1 $\pm$ 0.4 $\%$} & {\color{brown} 0.1 $\pm$ 0.0 $\%$} & {\color{brown} 0.3 $\pm$ 0.2 $\%$}\\
        EasyMap & Expert & 0 $\%$
        & {\color{teal}R = 101.1 $\pm$ 0.0} & {\color{teal}R = 100.9 $\pm$ 1.7} & {\color{teal}R = 100.9 $\pm$ 0.6}\\
        & & & {\color{teal}S = 95.5 $\pm$ 0.7} & {\color{teal}S = 95.5 $\pm$ 0.7} & {\color{teal}S = 94.3 $\pm$ 0.5}\\

        \hline

        % Easy-intermediate
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 101.4 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ R = 101.9 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ R = 99.9 $\pm$ 1.0 \\
        
        \hline
        
        & & & {\color{brown} 15.4 $\pm$ 0.3 $\%$} & {\color{brown} 26.4 $\pm$ 0.5 $\%$} & {\color{brown} 21.4 $\pm$ 0.9 $\%$}\\
        EasyMap & Intermediate & 50 $\%$
        & {\color{teal}R = 99.2 $\pm$ 0.5} & {\color{teal}R = 101.3 $\pm$ 0.2} & {\color{teal}R = 99.7 $\pm$ 2.2}\\
        & & & {\color{teal}S = 94.0 $\pm$ 0.7} & {\color{teal}S = 95.5 $\pm$ 0.2} & {\color{teal}S = 93.7 $\pm$ 2.8}\\
        
        \hline
        
        & & & {\color{brown} 9.3 $\pm$ 0.2 $\%$} & {\color{brown} 7.8 $\pm$ 0.5 $\%$} & {\color{brown} 7.4 $\pm$ 0.6 $\%$}\\
        EasyMap & Intermediate & 10 $\%$
        & {\color{teal}R = 99.9 $\pm$ 0.1} & {\color{teal}R = 101.5 $\pm$ 0.2} & {\color{teal}R = 98.7 $\pm$ 0.6}\\
        & & & {\color{teal}S = 94.7 $\pm$ 0.1} & {\color{teal}S = 95.5 $\pm$ 0.2} & {\color{teal}S = 93.3 $\pm$ 0.9}\\
        
        \hline
        
        & & & {\color{brown} 2.6 $\pm$ 0.3 $\%$} & {\color{brown} 1.0 $\pm$ 0.0 $\%$} & {\color{brown} 1.2 $\pm$ 0.0 $\%$}\\
        EasyMap & Intermediate & 1 $\%$
        & {\color{teal}R = 99.4 $\pm$ 0.5} & {\color{teal}R = 99.0 $\pm$ 1.1} & {\color{teal}R = 99.4 $\pm$ 0.2}\\
        & & & {\color{teal}S = 94.5 $\pm$ 0.5} & {\color{teal}S = 93.8 $\pm$ 1.2} & {\color{teal}S = 93.3 $\pm$ 0.0}\\
        
        \hline
        
        & & & {\color{brown} 2.1 $\pm$ 0.4 $\%$} & {\color{brown} 0.4 $\pm$ 0.0 $\%$} & {\color{brown} 0.5 $\pm$ 0.1 $\%$}\\
        EasyMap & Intermediate & 0 $\%$
        & {\color{teal}R = 98.7 $\pm$ 0.0} & {\color{teal}R = 99.0 $\pm$ 1.7} & {\color{teal}R = 99.4 $\pm$ 0.6}\\
        & & & {\color{teal}S = 93.7 $\pm$ 0.0} & {\color{teal}S = 93.8 $\pm$ 1.6} & {\color{teal}S = 92.5 $\pm$ 0.7}\\

        \hline

        % Hard-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 82.7 $\pm$ 1.0
            & 100.0 $\%$ $\vert$\ R = 76.2 $\pm$ 1.0
            & 100.0 $\%$ $\vert$\ R = 77.6 $\pm$ 1.2 \\
        
        \hline
        
        & & & {\color{brown} 27.1 $\pm$ 1.1 $\%$} & {\color{brown} 36.4 $\pm$ 0.4 $\%$} & {\color{brown} 30.7 $\pm$ 0.4 $\%$}\\
        HardMap & Expert & 50 $\%$
        & {\color{teal}R = 82.4 $\pm$ 2.3} & {\color{teal}R = 74.9 $\pm$ 0.5} & {\color{teal}R = 72.1 $\pm$ 1.0}\\
        & & & {\color{teal}S = 80.0 $\pm$ 3.3} & {\color{teal}S = 70.0 $\pm$ 0.5} & {\color{teal}S = 66.8 $\pm$ 0.2}\\
        
        \hline
        
        & & & {\color{brown} 10.2 $\pm$ 0.1 $\%$} & {\color{brown} 7.7 $\pm$ 0.2 $\%$} & {\color{brown} 7.2 $\pm$ 0.2 $\%$}\\
        HardMap & Expert & 10 $\%$
        & {\color{teal}R = 78.8 $\pm$ 2.4} & {\color{teal}R = 72.5 $\pm$ 5.1} & {\color{teal}R = 70.1 $\pm$ 0.2}\\
        & & & {\color{teal}S = 77.3 $\pm$ 1.4} & {\color{teal}S = 68.3 $\pm$ 1.9} & {\color{teal}S = 65.3 $\pm$ 0.9}\\

        \hline
        
        & & & {\color{brown} 2.9 $\pm$ 0.0 $\%$} & {\color{brown} 0.8 $\pm$ 0.1 $\%$} & {\color{brown} 0.9 $\pm$ 0.2 $\%$}\\
        HardMap & Expert & 1 $\%$
        & {\color{teal}R = 71.6 $\pm$ 1.5} & {\color{teal}R = 53.0 $\pm$ 5.5} & {\color{teal}R = 56.7 $\pm$ 1.5}\\
        & & & {\color{teal}S = 70.2 $\pm$ 2.1} & {\color{teal}S = 53.5 $\pm$ 7.3} & {\color{teal}S = 54.3 $\pm$ 0.5}\\

        \hline
        
        & & & {\color{brown} 1.9 $\pm$ 0.0 $\%$} & {\color{brown} 0.3 $\pm$ 0.2 $\%$} & {\color{brown} 0.4 $\pm$ 0.0 $\%$}\\
        HardMap & Expert & 0 $\%$
        & {\color{teal}R = 68.7 $\pm$ 4.7} & {\color{teal}R = 46.9 $\pm$ 2.2} & {\color{teal}R = 45.0 $\pm$ 2.6}\\
        & & & {\color{teal}S = 69.3 $\pm$ 3.3} & {\color{teal}S = 46.5 $\pm$ 2.6} & {\color{teal}S = 44.2 $\pm$ 1.2}\\

        \hline

        % Hard-intermediate
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 52.2 $\pm$ 1.7
            & 100.0 $\%$ $\vert$\ R = 50.2 $\pm$ 1.3
            & 100.0 $\%$ $\vert$\ R = 46.7 $\pm$ 1.4 \\
        
        \hline
        
        & & & {\color{brown} 27.1 $\pm$ 0.3 $\%$} & {\color{brown} 36.4 $\pm$ 0.2 $\%$} & {\color{brown} 30.7 $\pm$ 0.1 $\%$}\\
        HardMap & Intermediate & 50 $\%$
        & {\color{teal}R = 51.0 $\pm$ 0.5} & {\color{teal}R = 49.9 $\pm$ 1.3} & {\color{teal}R = 45.3 $\pm$ 0.5}\\
        & & & {\color{teal}S = 45.5 $\pm$ 0.7} & {\color{teal}S = 43.2 $\pm$ 0.2} & {\color{teal}S = 38.3 $\pm$ 0.9}\\
        
        \hline
        
        & & & {\color{brown} 9.6 $\pm$ 0.0 $\%$} & {\color{brown} 9.5 $\pm$ 0.7 $\%$} & {\color{brown} 8.8 $\pm$ 0.5 $\%$}\\
        HardMap & Intermediate & 10 $\%$
        & {\color{teal}R = 52.5 $\pm$ 0.9} & {\color{teal}R = 49.4 $\pm$ 1.2} & {\color{teal}R = 44.7 $\pm$ 0.8}\\
        & & & {\color{teal}S = 46.5 $\pm$ 0.2} & {\color{teal}S = 43.7 $\pm$ 2.8} & {\color{teal}S = 37.2 $\pm$ 0.7}\\

        \hline
        
        & & & {\color{brown} 1.9 $\pm$ 0.0 $\%$} & {\color{brown} 1.7 $\pm$ 0.0 $\%$} & {\color{brown} 1.6 $\pm$ 0.1 $\%$}\\
        HardMap & Intermediate & 1 $\%$
        & {\color{teal}R = 48.9 $\pm$ 0.4} & {\color{teal}R = 40.7 $\pm$ 0.5} & {\color{teal}R = 40.7 $\pm$ 1.4}\\
        & & & {\color{teal}S = 45.4 $\pm$ 2.3} & {\color{teal}S = 37.3 $\pm$ 0.5} & {\color{teal}S = 34.2 $\pm$ 0.7}\\

        \hline
        
        & & & {\color{brown} 1.2 $\pm$ 0.0 $\%$} & {\color{brown} 0.9 $\pm$ 0.0 $\%$} & {\color{brown} 1.2 $\pm$ 0.0 $\%$}\\
        HardMap & Intermediate & 0 $\%$
        & {\color{teal}R = 43.3 $\pm$ 3.0} & {\color{teal}R = 36.1 $\pm$ 0.3} & {\color{teal}R = 38.8 $\pm$ 0.2}\\
        & & & {\color{teal}S = 40.7 $\pm$ 2.8} & {\color{teal}S = 35.0 $\pm$ 0.9} & {\color{teal}S = 32.3 $\pm$ 0.5}\\

        \hline
    
    \end{tblr}
    \caption{{\color{brown}Average Cost} \& {\color{teal}Average Performance} on the 3D environments.}    
   \label{newbudget_rewards_godot}
\end{table*}

==> tables/new/baseline_d4rl.tex <==
\begin{table*}[!t]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|,
        row{1} = {pink},
        row{2-4} = {mygray},
        row{8-10} = {mygray},
        row{14-15} = {mydarkgray},
    }
        \hline
        \textbf{Dataset} & \textbf{Environment} & \textbf{DT} & \textbf{DT (original)} & \textbf{IQL} & \textbf{IQL (original)} & \textbf{RCBC} & \textbf{BC} \\
        \hline
        & HalfCheetah & 92.7 $\pm$ 0.1 & - & 91.6 $\pm$ 1.2 & - & 91.8 $\pm$ 0.7 & 92.5 $\pm$ 0.7 \\
        Expert & Hopper & 110.1 $\pm$ 1.6 & - & 89.7 $\pm$ 5.7 & - & 100.1 $\pm$ 15.2 & 110.9 $\pm$ 0.7 \\
        & Walker2D & 108.5 $\pm$ 0.8 & - & 110.5 $\pm$ 0.5 & - & 108.7 $\pm$ 0.1 & 108.8 $\pm$ 0.1 \\
        \hline
        & HalfCheetah & 92.5 $\pm$ 0.7 & 86.8 $\pm$ 1.3 & 87.9 $\pm$ 2.2 & 86.7 & 86.1 $\pm$ 3.1 & 49.5 $\pm$ 4.0 \\
        Medium-Expert & Hopper & 110.4 $\pm$ 0.8 & 107.6 $\pm$ 1.8 & 100.9 $\pm$ 7.8 & 91.5 & 89.4 $\pm$ 10.0 & 49.8 $\pm$ 6.1 \\
        & Walker2D & 108.1 $\pm$ 1.3 & 108.1 $\pm$ 0.2 & 109.1 $\pm$ 2.8 & 109.6 & 95.1 $\pm$ 14.5 & 106.8 $\pm$ 2.4 \\
        \hline
        & HalfCheetah & 42.7 $\pm$ 0.2 & 42.6 $\pm$ 0.1 & 47.3 $\pm$ 0.2 & 47.4 & 42.7 $\pm$ 0.3 & 42.3 $\pm$ 0.2 \\
        Medium & Hopper & 65.0 $\pm$ 4.7 & 67.6 $\pm$ 1.0 & 88.0 $\pm$ 12.4 & 66.3 & 63.4 $\pm$ 3.5 & 54.5 $\pm$ 2.1 \\
        & Walker2D & 74.1 $\pm$ 0.8 & 74.0 $\pm$ 1.4 & 78.0 $\pm$ 1.9 & 78.3 & 74.2 $\pm$ 1.4 & 71.2 $\pm$ 2.0 \\
        \hline
        & HalfCheetah & 40.5 $\pm$ 0.8 & 36.6 $\pm$ 0.8 & 44.4 $\pm$ 0.2 & 44.2 & 37.0 $\pm$ 1.5 & 35.8 $\pm$ 2.6 \\
        Medium-Replay & Hopper & 77.1 $\pm$ 18.4 & 82.7 $\pm$ 7.0 & 88.1 $\pm$ 11.9 & 94.7 & 32.0 $\pm$ 26.5 & 28.9 $\pm$ 1.6 \\
        & Walker2D & 69.4 $\pm$ 3.3 & 66.6 $\pm$ 3.0 & 74.6 $\pm$ 7.7 & 73.9 & 46.5 $\pm$ 31.0 & 17.7 $\pm$ 5.7 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average (Without Expert)} & & 75.5 & 74.7 & 79.8 & 76.9 & 62.9 & 50.7 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average (With Expert)} & & 82.6 & - & 84.2 & - & 72.3 & 64.1 \\
        \hline
    \end{tblr}
    \caption{\textbf{\textcolor{red}{OLD RESULTS}} Average normalized cumulative rewards for query-free models on OpenAI Gym environments.\\
    These experiments allow us to validate the action component implementation of each model,
    as DT and IQL achieve
    close performances to the original papers,
    and to set the baseline for a quantitative study of our different budgeted models.}
\label{old_baseline_rewards_d4rl}
\end{table*}




\begin{table*}[!b]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|c|,
        row{1-2} = {pink},
        row{3-5} = {mygray},
        row{9-11} = {mygray},
        row{15-16} = {mydarkgray},
    }
        \hline
        \textbf{Dataset} & \textbf{Environment} & \textbf{DT} & \textbf{DT} & \textbf{DT} & \textbf{IQL} & \textbf{IQL} & \textbf{RCBC} & \textbf{RCBC} & \textbf{BC} \\
        & & \textbf{(RTG)} & \textbf{(No RTG)} & \textbf{(Original)} & & \textbf{(Original)} & \textbf{(RTG)} & \textbf{(No RTG)} & \\
        \hline
        & HalfCheetah & 92.4 $\pm$ 0.5 & 92.6 $\pm$ 0.4 & - & 91.4 $\pm$ 2.3 & - & 92.5 $\pm$ 0.2 & 92.7 $\pm$ 0.2 & 93.0 $\pm$ 0.2 \\
        Expert & Hopper & 110.4 $\pm$ 0.6 & 108.3 $\pm$ 4.9 & - & 98.3 $\pm$ 7.9 & - & 109.9 $\pm$ 0.9 & 109.8 $\pm$ 1.5 & 111.0 $\pm$ 0.4 \\
        & Walker2D & 108.3 $\pm$ 0.3 & 108.5 $\pm$ 0.4 & - & 112.2 $\pm$ 2.1 & - & 108.8 $\pm$ 0.3 & 108.8 $\pm$ 0.1 & 108.9 $\pm$ 0.2 \\
        \hline
        & HalfCheetah & 92.5 $\pm$ 0.4 & 73.7 $\pm$ 7.0 & 86.8 $\pm$ 1.3 & 85.0 $\pm$ 5.6 & 86.7 & 89.9 $\pm$ 0.4 & 75.4 $\pm$ 2.8 & 45.7 $\pm$ 1.3 \\
        Medium-Expert & Hopper & 108.2 $\pm$ 4.4 & 83.9 $\pm$ 37.2 & 107.6 $\pm$ 1.8 & 100.1 $\pm$ 11.5 & 91.5 & 107.6 $\pm$ 1.6 & 54.9 $\pm$ 1.2 & 61.9 $\pm$ 3.9 \\
        & Walker2D & 108.5 $\pm$ 0.4 & 107.1 $\pm$ 1.6 & 108.1 $\pm$ 0.2 & 108.6 $\pm$ 2.3 & 109.6 & 107.3 $\pm$ 1.7 & 106.2 $\pm$ 1.9 & 108.6 $\pm$ 0.4 \\
        \hline
        & HalfCheetah & 42.5 $\pm$ 0.2 & 42.6 $\pm$ 0.1 & 42.6 $\pm$ 0.1 & 47.3 $\pm$ 0.3 & 47.4 & 42.7 $\pm$ 0.2 & 42.5 $\pm$ 0.1 & 42.6 $\pm$ 0.2 \\
        Medium & Hopper & 64.3 $\pm$ 4.2 & 51.6 $\pm$ 4.8 & 67.6 $\pm$ 1.0 & 77.6 $\pm$ 5.8 & 66.3 & 66.1 $\pm$ 2.6 & 56.9 $\pm$ 1.6 & 54.8 $\pm$ 1.4 \\
        & Walker2D & 71.0 $\pm$ 3.1 & 68.9 $\pm$ 6.2 & 74.0 $\pm$ 1.4 & 76.5 $\pm$ 3.1 & 78.3 & 75.2 $\pm$ 1.2 & 73.1 $\pm$ 1.4 & 73.2 $\pm$ 0.9 \\
        \hline
        & HalfCheetah & 38.0 $\pm$ 1.1 & 34.1 $\pm$ 1.5 & 36.6 $\pm$ 0.8 & 44.2 $\pm$ 0.3 & 44.2 & 38.1 $\pm$ 0.5 & 32.6 $\pm$ 2.8 & 34.7 $\pm$ 2.2 \\
        Medium-Replay & Hopper & 83.1 $\pm$ 8.4 & 29.3 $\pm$ 7.4 & 82.7 $\pm$ 7.0 & 93.3 $\pm$ 5.8 & 94.7 & 75.4 $\pm$ 11.0 & 28.2 $\pm$ 3.8 & 30.2 $\pm$ 1.6 \\
        & Walker2D & 68.2 $\pm$ 2.7 & 31.6 $\pm$ 6.0 & 66.6 $\pm$ 3.0 & 77.9 $\pm$ 2.4 & 73.9 & 66.7 $\pm$ 3.6 & 23.0 $\pm$ 21.4 & 31.3 $\pm$ 14.3 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average (Without Expert)} & & 75.1 & 58.1 & 74.7 & 78.9 & 76.9 & 74.3 & 54.8 & 53.7 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average (With Expert)} & & 82.3 & 69.4 & - & 84.4 & - & 81.7 & 67.0 & 66.3 \\
        \hline
    \end{tblr}
    \caption{\textbf{\textcolor{blue}{NEW RESULTS}} Average normalized cumulative rewards for query-free models on OpenAI Gym environments.\\
    These experiments allow us to validate the action component implementation of each model,
    as DT and IQL achieve
    close performances to the original papers,
    and to set the baseline for a quantitative study of our different budgeted models.}
\label{new_baseline_rewards_d4rl}
\end{table*}

==> tables/new/baseline_godot.tex <==
\newpage

\begin{table*}[!h]
    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|,
        row{1-2} = {pink},
        row{3-4} = {mygray},
        row{7-8} = {mygray},
        row{11-12} = {mydarkgray},
    }
        \hline
        \textbf{Dataset} & \textbf{Environment} & \textbf{DT} & \textbf{RCBC} & \textbf{BC} \\
        & & \textbf{(RTG)} & \textbf{(RTG)} & \textbf{BC} \\
        \hline
        Expert & EasyMap
        & R = 102.7 $\pm$ 0.8 & R = 101.1 $\pm$ 1.7 & R = 102.8 $\pm$ 0.1 \\
        & & - & - & - \\
        \hline
        Expert & HardMap 
        & R = 84.0 $\pm$ 0.5 & R = 72.4 $\pm$ 1.2 & R = 74.1 $\pm$ 1.0 \\
        & & - & - & - \\
        \hline
        Intermediate & EasyMap
        & R = 101.9 $\pm$ 1.0 & R = 102.5 $\pm$ 0.7 & R = 100.1 $\pm$ 0.1 \\
        & & - & - & - \\
        \hline
        Intermediate & HardMap
        & R = 53.1 $\pm$ 4.3 & R = 49.0 $\pm$ 0.6 & R = 46.0 $\pm$ 0.6 \\
        & & - & - & - \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average Reward}
        & & R = 85.5 & R = 81.3 & R = 80.8 \\
        \SetCell[c=2]{c}{Average Success}
        & & - & - & - \\
        \hline
    \end{tblr}
    \caption{\textbf{\textcolor{red}{OLD RESULTS}} Average normalized cumulative rewards (R) and Averaged success rate (S) for cost-free models on the 3D navigation environment without cost constraint. These experiments set the baseline for a quantitative study of our budgeted models.}
\label{old_baseline_rewards_godot}
\end{table*}

\begin{table*}[!h]
    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|,
        row{1-2} = {pink},
        row{3-4} = {mygray},
        row{7-8} = {mygray},
        row{11-12} = {mydarkgray},
    }
        \hline
        \textbf{Dataset} & \textbf{Environment} & \textbf{DT} & \textbf{DT} & \textbf{RCBC} & \textbf{RCBC} & \textbf{BC} \\
        & & \textbf{(RTG)} & \textbf{(No RTG)} & \textbf{(RTG)} & \textbf{(No RTG)} & \\
        \hline
        Expert & EasyMap
        & R = 102.6 $\pm$ 0.6 & R = 102.1 $\pm$ 0.3 & R = 101.9 $\pm$ 0.4 & R = 101.9 $\pm$ 0.4 & R = 101.6 $\pm$ 0.4 \\
        & & S = 79.6 $\pm$ 0.7 & S = 78.9 $\pm$ 0.4 & S = 70.9 $\pm$ 0.8 & S = 72.6 $\pm$ 0.5 & S = 72.6 $\pm$ 0.5 \\
        \hline
        Expert & HardMap 
        & R = 82.7 $\pm$ 1.0 & R = 80.8 $\pm$ 2.3 & R = 76.2 $\pm$ 1.0 & R = 76.8 $\pm$ 1.1 & R = 77.6 $\pm$ 1.2 \\
        & & S = 79.6 $\pm$ 0.9 & S = 78.9 $\pm$ 2.9 & S = 70.9 $\pm$ 0.6 & S = 72.6 $\pm$ 1.6 & S = 72.6 $\pm$ 1.1 \\
        \hline
        Intermediate & EasyMap
        & R = 101.4 $\pm$ 0.7 & R = 101.2 $\pm$ 0.3 & R = 101.9 $\pm$ 0.7 & R = 100.9 $\pm$ 0.5 & R = 99.9 $\pm$ 1.0 \\
        & & S = 96.5 $\pm$ 0.8 & S = 96.3 $\pm$ 0.3 & S = 96.9 $\pm$ 0.9 & S = 95.9 $\pm$ 0.6 & S = 94.3 $\pm$ 1.1 \\
        \hline
        Intermediate & HardMap
        & R = 52.2 $\pm$ 1.7 & R = 50.9 $\pm$ 0.9 & R = 50.2 $\pm$ 1.3 & R = 48.7 $\pm$ 0.9 & R = 46.7 $\pm$ 1.4 \\
        & & S = 47.3 $\pm$ 1.9 & S = 45.6 $\pm$ 1.0 & S = 43.5 $\pm$ 1.8 & S = 41.6 $\pm$ 1.0 & S = 39.5 $\pm$ 0.9 \\
        \hline
        \hline
        \SetCell[c=2]{c}{Average Reward}
        & & R = 84.7 & R = 83.8 & R = 82.6 & R = 82.1 & R = 81.4 \\
        \SetCell[c=2]{c}{Average Success}
        & & S = 80.0 & S = 79.2 & S = 76.7 & S = 76.4 & S = 75.4 \\
        \hline
    \end{tblr}
    \caption{\textbf{\textcolor{blue}{NEW RESULTS}} Average normalized cumulative rewards (R) and Averaged success rate (S) for cost-free models on the 3D navigation environment without cost constraint. These experiments set the baseline for a quantitative study of our budgeted models.}
\label{new_baseline_rewards_godot}
\end{table*}

==> tables/new/budget_d4rl_md.tex <==
\begin{table*}[h!]
    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{7} = {mydarkgray},
        row{12} = {mydarkgray},
        row{13-16} = {mygray},
        row{17-21} = {mydarkgray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
        \hline
        
        % halfcheetah-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 42.7 $\pm$ 0.2
            & 100.0 $\%$ $\vert$\ 47.3 $\pm$ 0.2 
            & 100.0 $\%$ $\vert$\ 42.7 $\pm$ 0.3
            & 100.0 $\%$ $\vert$\ 42.3 $\pm$ 0.2 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 98.5 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 42.4 $\pm$ 0.2}
            & {\color{brown} 99.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 47.1 $\pm$ 0.1}
            & {\color{brown} 99.8 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.3 $\pm$ 0.2}
            & {\color{brown} 99.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.2 $\pm$ 0.1} \\
        Medium & HalfCheetah & 75 $\%$
            & {\color{brown} 71.5 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 42.5 $\pm$ 0.2}
            & {\color{brown} 75.1 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 46.6 $\pm$ 0.2}
            & {\color{brown} 70.0 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 39.7 $\pm$ 0.2}
            & {\color{brown} 69.7 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 39.7 $\pm$ 0.5} \\
        & & 50 $\%$
            & {\color{brown} 47.8 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 37.5 $\pm$ 1.8}
            & {\color{brown} 65.8 $\pm$ 1.6 $\%$} $\vert$\ {\color{teal} 45.6 $\pm$ 0.7}
            & {\color{brown} 47.6 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 29.7 $\pm$ 1.3}
            & {\color{brown} 48.4 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 31.3 $\pm$ 0.7} \\
        & & 25 $\%$
            & {\color{brown} 33.3 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 28.8 $\pm$ 5.5}
            & {\color{brown} 64.6 $\pm$ 2.0 $\%$} $\vert$\ {\color{teal} 45.6 $\pm$ 0.8}
            & {\color{brown} 35.1 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 22.7 $\pm$ 0.4}
            & {\color{brown} 37.9 $\pm$ 0.9 $\%$} $\vert$\ {\color{teal} 21.2 $\pm$ 2.2} \\

        \hline

        % hopper-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 65.0 $\pm$ 4.7
            & 100.0 $\%$ $\vert$\ 88.0 $\pm$ 12.4 
            & 100.0 $\%$ $\vert$\ 63.4 $\pm$ 3.5
            & 100.0 $\%$ $\vert$\ 54.5 $\pm$ 2.1 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 85.1 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 61.8 $\pm$ 7.8}
            & {\color{brown} 93.3 $\pm$ 4.3 $\%$} $\vert$\ {\color{teal} 62.5 $\pm$ 6.1}
            & {\color{brown} 99.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 69.2 $\pm$ 4.7}
            & {\color{brown} 98.8 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 52.7 $\pm$ 1.9} \\
        Medium & Hopper & 75 $\%$
            & {\color{brown} 79.9 $\pm$ 2.2 $\%$} $\vert$\ {\color{teal} 52.0 $\pm$ 5.4}
            & {\color{brown} 68.7 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 45.3 $\pm$ 8.0}
            & {\color{brown} 71.7 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 45.4 $\pm$ 8.9}
            & {\color{brown} 66.6 $\pm$ 2.1 $\%$} $\vert$\ {\color{teal} 39.1 $\pm$ 1.7} \\
        & & 50 $\%$
            & {\color{brown} 68.1 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 60.5 $\pm$ 0.5}
            & {\color{brown} 43.5 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 14.2 $\pm$ 1.8}
            & {\color{brown} 43.9 $\pm$ 0.9 $\%$} $\vert$\ {\color{teal} 23.7 $\pm$ 4.4}
            & {\color{brown} 42.6 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 25.5 $\pm$ 3.5} \\
        & & 25 $\%$
            & {\color{brown} 51.0 $\pm$ 1.3 $\%$} $\vert$\ {\color{teal} 68.1 $\pm$ 19.8}
            & {\color{brown} 18.1 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 7.6 $\pm$ 0.9}
            & {\color{brown} 19.9 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 8.6 $\pm$ 1.5}
            & {\color{brown} 22.0 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 4.3 $\pm$ 0.3} \\

        \hline

        % walker2d-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 74.1 $\pm$ 0.8
            & 100.0 $\%$ $\vert$\ 78.0 $\pm$ 1.9 
            & 100.0 $\%$ $\vert$\ 74.2 $\pm$ 1.4
            & 100.0 $\%$ $\vert$\ 71.2 $\pm$ 2.0 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 97.0 $\pm$ 2.8 $\%$} $\vert$\ {\color{teal} 61.4 $\pm$ 12.9}
            & {\color{brown} 99.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 73.2 $\pm$ 2.9}
            & {\color{brown} 99.8 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 73.6 $\pm$ 1.6}
            & {\color{brown} 99.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 71.0 $\pm$ 1.2} \\
        Medium & Walker2D & 75 $\%$
            & {\color{brown} 74.2 $\pm$ 0.9 $\%$} $\vert$\ {\color{teal} 66.3 $\pm$ 11.7}
            & {\color{brown} 71.9 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 37.5 $\pm$ 12.2}
            & {\color{brown} 70.5 $\pm$ 1.2 $\%$} $\vert$\ {\color{teal} 67.7 $\pm$ 2.1}
            & {\color{brown} 68.8 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 56.4 $\pm$ 4.0} \\
        & & 50 $\%$
            & {\color{brown} 48.2 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 62.5 $\pm$ 0.0}
            & {\color{brown} 55.4 $\pm$ 0.9 $\%$} $\vert$\ {\color{teal} 6.0 $\pm$ 2.1}
            & {\color{brown} 44.3 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 21.0 $\pm$ 6.0}
            & {\color{brown} 45.9 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 19.5 $\pm$ 5.3} \\
        & & 25 $\%$
            & {\color{brown} 32.7 $\pm$ 5.5 $\%$} $\vert$\ {\color{teal} 0.4 $\pm$ 0.2}
            & {\color{brown} 47.1 $\pm$ 2.5 $\%$} $\vert$\ {\color{teal} 5.8 $\pm$ 1.1}
            & {\color{brown} 28.4 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 9.5 $\pm$ 1.5}
            & {\color{brown} 31.8 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 11.5 $\pm$ 0.6} \\

        \hline
        \hline
        \SetCell[c=2]{c}{} & & baseline
            & 100.0 $\%$ $\vert$\ 60.6
            & 100.0 $\%$ $\vert$\ 71.1
            & 100.0 $\%$ $\vert$\ 60.1
            & 100.0 $\%$ $\vert$\ 56.0 \\
        \hline
        \SetCell[c=2]{c}{} & & 100 $\%$
            & {\color{brown} 93.5 $\%$} $\vert$\ {\color{teal} 55.2}
            & {\color{brown} 97.4 $\%$} $\vert$\ {\color{teal} 60.9}
            & {\color{brown} 99.7 $\%$} $\vert$\ {\color{teal} 61.7}
            & {\color{brown} 98.4 $\%$} $\vert$\ {\color{teal} 55.3} \\
        \SetCell[c=2]{c}{Average} & & 75 $\%$
            & {\color{brown} 75.2 $\%$} $\vert$\ {\color{teal} 53.6}
            & {\color{brown} 71.9 $\%$} $\vert$\ {\color{teal} 43.1}
            & {\color{brown} 70.7 $\%$} $\vert$\ {\color{teal} 50.9}
            & {\color{brown} 68.4 $\%$} $\vert$\ {\color{teal} 45.1} \\
        \SetCell[c=2]{c}{} & & 50 $\%$
            & {\color{brown} 54.7 $\%$} $\vert$\ {\color{teal} 53.5}
            & {\color{brown} 54.9 $\%$} $\vert$\ {\color{teal} 21.9}
            & {\color{brown} 45.3 $\%$} $\vert$\ {\color{teal} 24.8}
            & {\color{brown} 45.6 $\%$} $\vert$\ {\color{teal} 25.4} \\
        \SetCell[c=2]{c}{} & & 25 $\%$
            & {\color{brown} 39.0 $\%$} $\vert$\ {\color{teal} 32.4}
            & {\color{brown} 43.3 $\%$} $\vert$\ {\color{teal} 19.7}
            & {\color{brown} 27.8 $\%$} $\vert$\ {\color{teal} 13.6}
            & {\color{brown} 30.6 $\%$} $\vert$\ {\color{teal} 12.3} \\

        \hline
        
    \end{tblr}
    \caption{\textbf{\textcolor{red}{OLD RESULTS}} {\color{brown}Average Cost} \& {\color{teal}Average Performance} on D4RL environments for the \textbf{Medium  datasets}.}
\label{old_budget_rewards_d4rl_md}
\end{table*}




\begin{table*}[h!]
    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{7} = {mydarkgray},
        row{12} = {mydarkgray},
        row{13-16} = {mygray},
        row{17-21} = {mydarkgray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % halfcheetah-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 42.5 $\pm$ 0.2
            & 100.0 $\%$ $\vert$\ 47.3 $\pm$ 0.3 
            & 100.0 $\%$ $\vert$\ 42.7 $\pm$ 0.2
            & 100.0 $\%$ $\vert$\ 42.6 $\pm$ 1.3 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 98.9 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 42.9 $\pm$ 0.1}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 47.1 $\pm$ 0.4}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.6 $\pm$ 0.2}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.7 $\pm$ 0.2} \\
        Medium & Halfcheetah & 75 $\%$
            & {\color{brown} 67.2 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 42.6 $\pm$ 0.1}
            & {\color{brown} 81.2 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 47.4 $\pm$ 0.2}
            & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.7 $\pm$ 0.1}
            & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.5 $\pm$ 0.6} \\
        & & 50 $\%$
            & {\color{brown} 44.1 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 40.9 $\pm$ 0.6}
            & {\color{brown} 70.6 $\pm$ 7.2 $\%$} $\vert$\ {\color{teal} 47.7 $\pm$ 0.4}
            & {\color{brown} 55.3 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 40.8 $\pm$ 0.9}
            & {\color{brown} 56.3 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 41.6 $\pm$ 1.2} \\
        & & 25 $\%$
            & {\color{brown} 24.0 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 30.5 $\pm$ 1.9}
            & {\color{brown} 61.2 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 47.7 $\pm$ 0.2}
            & {\color{brown} 23.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 10.9 $\pm$ 0.9}
            & {\color{brown} 28.2 $\pm$ 4.9 $\%$} $\vert$\ {\color{teal} 16.9 $\pm$ 4.6} \\

        \hline

        % hopper-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 64.3 $\pm$ 4.2
            & 100.0 $\%$ $\vert$\ 77.6 $\pm$ 5.8 
            & 100.0 $\%$ $\vert$\ 66.1 $\pm$ 2.6
            & 100.0 $\%$ $\vert$\ 54.8 $\pm$ 1.4 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 92.6 $\pm$ 1.7 $\%$} $\vert$\ {\color{teal} 66.4 $\pm$ 1.6}
            & {\color{brown} 94.5 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 72.7 $\pm$ 6.0}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 69.5 $\pm$ 3.5}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 56.0 $\pm$ 0.6} \\
        Medium & Hopper & 75 $\%$
            & {\color{brown} 64.9 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 87.4 $\pm$ 1.5}
            & {\color{brown} 74.5 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 74.5 $\pm$ 14.9}
            & {\color{brown} 69.1 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 55.8 $\pm$ 10.6}
            & {\color{brown} 74.5 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 47.5 $\pm$ 2.5} \\
        & & 50 $\%$
            & {\color{brown} 37.5 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 29.1 $\pm$ 12.8}
            & {\color{brown} 52.7 $\pm$ 7.6 $\%$} $\vert$\ {\color{teal} 11.9 $\pm$ 7.7}
            & {\color{brown} 45.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 40.5 $\pm$ 9.7}
            & {\color{brown} 36.4 $\pm$ 9.1 $\%$} $\vert$\ {\color{teal} 8.4 $\pm$ 4.8} \\
        & & 25 $\%$
            & {\color{brown} 17.7 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 13.7 $\pm$ 2.8}
            & {\color{brown} 12.7 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 5.2 $\pm$ 2.4}
            & {\color{brown} 18.2 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 8.3 $\pm$ 3.7}
            & {\color{brown} 16.4 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 4.5 $\pm$ 2.4} \\

        \hline

        %walker2d-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 71.0 $\pm$ 3.1
            & 100.0 $\%$ $\vert$\ 76.5 $\pm$ 3.1 
            & 100.0 $\%$ $\vert$\ 75.2 $\pm$ 1.2
            & 100.0 $\%$ $\vert$\ 73.2 $\pm$ 0.9 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 99.3 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 75.3 $\pm$ 1.3}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 77.8 $\pm$ 7.6}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 73.7 $\pm$ 2.0}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 73.0 $\pm$ 1.4} \\
        Medium & Walker2D & 75 $\%$
            & {\color{brown} 67.3 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 72.7 $\pm$ 5.3}
            & {\color{brown} 80.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 62.7 $\pm$ 25.5}
            & {\color{brown} 74.1 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 71.6 $\pm$ 4.1}
            & {\color{brown} 76.5 $\pm$ 4.2 $\%$} $\vert$\ {\color{teal} 69.1 $\pm$ 4.6} \\
        & & 50 $\%$
            & {\color{brown} 46.0 $\pm$ 2.5 $\%$} $\vert$\ {\color{teal} 17.4 $\pm$ 5.7}
            & {\color{brown} 62.4 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 17.0 $\pm$ 4.4}
            & {\color{brown} 56.5 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 30.5 $\pm$ 15.5}
            & {\color{brown} 52.9 $\pm$ 4.2 $\%$} $\vert$\ {\color{teal} 14.6 $\pm$ 14.0} \\
        & & 25 $\%$
            & {\color{brown} 19.0 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 1.3 $\pm$ 0.4}
            & {\color{brown} 42.4 $\pm$ 4.9 $\%$} $\vert$\ {\color{teal} 6.4 $\pm$ 1.3}
            & {\color{brown} 20.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 6.6 $\pm$ 1.2}
            & {\color{brown} 21.2 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 4.4 $\pm$ 3.0} \\

        \hline
        \hline
        \SetCell[c=2]{c}{} & & baseline
            & 100.0 $\%$ $\vert$\ 59.3
            & 100.0 $\%$ $\vert$\ 67.1
            & 100.0 $\%$ $\vert$\ 61.3
            & 100.0 $\%$ $\vert$\ 56.9 \\
        \hline
        \SetCell[c=2]{c}{} & & 100 $\%$
            & {\color{brown} 98.2 $\%$} $\vert$\ {\color{teal} 61.7}
            & {\color{brown} 98.2 $\%$} $\vert$\ {\color{teal} 64.5}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 61.5}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 56.6} \\
        \SetCell[c=2]{c}{Average} & & 75 $\%$
            & {\color{brown} 66.9 $\%$} $\vert$\ {\color{teal} 69.3}
            & {\color{brown} 78.6 $\%$} $\vert$\ {\color{teal} 59.6}
            & {\color{brown} 73.2 $\%$} $\vert$\ {\color{teal} 55.7}
            & {\color{brown} 75.8 $\%$} $\vert$\ {\color{teal} 51.1} \\
        \SetCell[c=2]{c}{} & & 50 $\%$
            & {\color{brown} 43.9 $\%$} $\vert$\ {\color{teal} 27.7}
            & {\color{brown} 61.9 $\%$} $\vert$\ {\color{teal} 24.9}
            & {\color{brown} 52.4 $\%$} $\vert$\ {\color{teal} 34.2}
            & {\color{brown} 48.2 $\%$} $\vert$\ {\color{teal} 20.7} \\
        \SetCell[c=2]{c}{} & & 25 $\%$
            & {\color{brown} 20.5 $\%$} $\vert$\ {\color{teal} 14.7}
            & {\color{brown} 37.8 $\%$} $\vert$\ {\color{teal} 19.5}
            & {\color{brown} 20.6 $\%$} $\vert$\ {\color{teal} 8.2}
            & {\color{brown} 20.7 $\%$} $\vert$\ {\color{teal} 8.0} \\

        \hline
        
    \end{tblr}
    \caption{\textbf{\textcolor{blue}{NEW RESULTS}} {\color{brown}Average Cost} \& {\color{teal}Average Performance} on D4RL environments for the \textbf{Medium  datasets}.}
\label{new_budget_rewards_d4rl_md}
\end{table*}

==> tables/new/budget_d4rl_xp.tex <==
\begin{table*}[!h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{7} = {mydarkgray},
        row{12} = {mydarkgray},
        row{13-16} = {mygray},
        row{17-21} = {mydarkgray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1
            & 100.0 $\%$ $\vert$\ 91.6 $\pm$ 1.2 
            & 100.0 $\%$ $\vert$\ 92.1 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 95.3 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 90.0 $\pm$ 2.3}
            & {\color{brown} 93.0 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 75.1 $\pm$ 6.5}
            & {\color{brown} 99.8 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 89.2 $\pm$ 0.3}
            & {\color{brown} 99.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 89.5 $\pm$ 0.6} \\
        Expert & HalfCheetah & 75 $\%$
            & {\color{brown} 72.5 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 87.8 $\pm$ 0.6}
            & {\color{brown} 71.0 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 56.7 $\pm$ 5.9}
            & {\color{brown} 72.0 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 68.6 $\pm$ 2.1}
            & {\color{brown} 70.8 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 66.6 $\pm$ 7.6} \\
        & & 50 $\%$
            & {\color{brown} 48.9 $\pm$ 1.4 $\%$} $\vert$\ {\color{teal} 69.5 $\pm$ 15.2}
            & {\color{brown} 55.0 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 16.4 $\pm$ 0.4}
            & {\color{brown} 46.6 $\pm$ 1.3 $\%$} $\vert$\ {\color{teal} 16.9 $\pm$ 8.1}
            & {\color{brown} 45.1 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 13.1 $\pm$ 2.2} \\
        & & 25 $\%$
            & {\color{brown} 27.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 56.3 $\pm$ 0.0}
            & {\color{brown} 52.3 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 11.7 $\pm$ 0.6}
            & {\color{brown} 27.0 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 4.7 $\pm$ 0.9}
            & {\color{brown} 28.0 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 4.9 $\pm$ 0.4} \\

        \hline

        % hopper-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6
            & 100.0 $\%$ $\vert$\ 89.7 $\pm$ 5.7 
            & 100.0 $\%$ $\vert$\ 100.1 $\pm$ 15.2
            & 100.0 $\%$ $\vert$\ 110.9 $\pm$ 0.7 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 84.6 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 82.6 $\pm$ 21.3}
            & {\color{brown} 98.2 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 57.1 $\pm$ 32.3}
            & {\color{brown} 99.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 100.0 $\pm$ 10.8}
            & {\color{brown} 99.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 98.0 $\pm$ 13.5} \\
        Expert & Hopper & 75 $\%$
            & {\color{brown} 71.3 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 70.2 $\pm$ 43.5}
            & {\color{brown} 71.5 $\pm$ 2.1 $\%$} $\vert$\ {\color{teal} 26.9 $\pm$ 8.5}
            & {\color{brown} 72.5 $\pm$ 1.2 $\%$} $\vert$\ {\color{teal} 88.4 $\pm$ 5.4}
            & {\color{brown} 68.0 $\pm$ 3.3 $\%$} $\vert$\ {\color{teal} 66.0 $\pm$ 19.1} \\
        & & 50 $\%$
            & {\color{brown} 49.1 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 54.0 $\pm$ 11.5}
            & {\color{brown} 44.2 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 5.4 $\pm$ 4.0}
            & {\color{brown} 43.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 25.5 $\pm$ 4.8}
            & {\color{brown} 40.6 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 21.2 $\pm$ 2.7} \\
        & & 25 $\%$
            & {\color{brown} 29.0 $\pm$ 2.1 $\%$} $\vert$\ {\color{teal} 13.5 $\pm$ 3.2}
            & {\color{brown} 20.3 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 3.5 $\pm$ 2.3}
            & {\color{brown} 18.3 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 16.0 $\pm$ 2.3}
            & {\color{brown} 19.8 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 5.8 $\pm$ 1.5} \\

        \hline

        %walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.5 $\pm$ 0.8
            & 100.0 $\%$ $\vert$\ 110.5 $\pm$ 0.5
            & 100.0 $\%$ $\vert$\ 108.7 $\pm$ 0.1
            & 100.0 $\%$ $\vert$\ 108.8 $\pm$ 0.1 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 93.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 107.5 $\pm$ 0.0}
            & {\color{brown} 88.3 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 99.9 $\pm$ 6.6}
            & {\color{brown} 99.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.2 $\pm$ 0.3}
            & {\color{brown} 99.3 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.4 $\pm$ 0.2} \\
        Expert & Walker2D & 75 $\%$
            & {\color{brown} 73.5 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 104.7 $\pm$ 4.1}
            & {\color{brown} 74.4 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 96.8 $\pm$ 6.4}
            & {\color{brown} 74.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 106.2 $\pm$ 2.4}
            & {\color{brown} 73.1 $\pm$ 1.0 $\%$} $\vert$\ {\color{teal} 106.4 $\pm$ 0.3} \\
        & & 50 $\%$
            & {\color{brown} 50.7 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 82.8 $\pm$ 13.4}
            & {\color{brown} 45.4 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 9.1 $\pm$ 2.2}
            & {\color{brown} 44.6 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 23.4 $\pm$ 2.8}
            & {\color{brown} 43.5 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 15.2 $\pm$ 2.2} \\
        & & 25 $\%$
            & {\color{brown} 27.0 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 21.8 $\pm$ 12.9}
            & {\color{brown} 23.4 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 4.6 $\pm$ 1.5}
            & {\color{brown} 24.8 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 10.1 $\pm$ 0.9}
            & {\color{brown} 29.0 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 6.7 $\pm$ 0.4} \\

        \hline
        \hline
        \SetCell[c=2]{c}{} & & baseline
            & 100.0 $\%$ $\vert$\ 103.8
            & 100.0 $\%$ $\vert$\ 97.3
            & 100.0 $\%$ $\vert$\ 100.3
            & 100.0 $\%$ $\vert$\ 104.1 \\
        \hline
        \SetCell[c=2]{c}{} & & 100 $\%$
            & {\color{brown} 91.1 $\%$} $\vert$\ {\color{teal} 93.4}
            & {\color{brown} 93.2 $\%$} $\vert$\ {\color{teal} 77.4}
            & {\color{brown} 99.6 $\%$} $\vert$\ {\color{teal} 99.1}
            & {\color{brown} 99.3 $\%$} $\vert$\ {\color{teal} 98.6} \\
        \SetCell[c=2]{c}{Average} & & 75 $\%$
            & {\color{brown} 72.4 $\%$} $\vert$\ {\color{teal} 87.6}
            & {\color{brown} 72.3 $\%$} $\vert$\ {\color{teal} 60.1}
            & {\color{brown} 73.0 $\%$} $\vert$\ {\color{teal} 87.7}
            & {\color{brown} 70.6 $\%$} $\vert$\ {\color{teal} 79.7} \\
        \SetCell[c=2]{c}{} & & 50 $\%$
            & {\color{brown} 49.6 $\%$} $\vert$\ {\color{teal} 68.8}
            & {\color{brown} 48.2 $\%$} $\vert$\ {\color{teal} 10.3}
            & {\color{brown} 44.7 $\%$} $\vert$\ {\color{teal} 21.9}
            & {\color{brown} 43.1 $\%$} $\vert$\ {\color{teal} 16.5} \\
        \SetCell[c=2]{c}{} & & 25 $\%$
            & {\color{brown} 27.2 $\%$} $\vert$\ {\color{teal} 30.5}
            & {\color{brown} 33.0 $\%$} $\vert$\ {\color{teal} 6.6}
            & {\color{brown} 25.5 $\%$} $\vert$\ {\color{teal} 10.3}
            & {\color{brown} 28.7 $\%$} $\vert$\ {\color{teal} 5.8} \\

        \hline
        
    \end{tblr}
    \caption{\textbf{\textcolor{red}{OLD RESULTS}} {\color{brown}Average Cost} \& {\color{teal}Average Performance} on D4RL environments for the \textbf{Expert  datasets}.}    
   \label{old_budget_rewards_d4rl_xp}
\end{table*}




\begin{table*}[!h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{7} = {mydarkgray},
        row{12} = {mydarkgray},
        row{13-16} = {mygray},
        row{17-21} = {mydarkgray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.4 $\pm$ 0.5
            & 100.0 $\%$ $\vert$\ 91.4 $\pm$ 2.3 
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.2
            & 100.0 $\%$ $\vert$\ 93.0 $\pm$ 0.2 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 97.5 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 92.4 $\pm$ 0.5}
            & {\color{brown} 97.6 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 85.9 $\pm$ 6.9}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 92.3 $\pm$ 0.2}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 93.0 $\pm$ 0.2} \\
        Expert & HalfCheetah & 75 $\%$
            & {\color{brown} 64.8 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 89.1 $\pm$ 1.2}
            & {\color{brown} 80.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 74.2 $\pm$ 3.9}
            & {\color{brown} 70.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 89.1 $\pm$ 1.1}
            & {\color{brown} 75.3 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 90.1 $\pm$ 1.0} \\
        & & 50 $\%$
            & {\color{brown} 44.5 $\pm$ 1.4 $\%$} $\vert$\ {\color{teal} 72.8 $\pm$ 6.5}
            & {\color{brown} 63.5 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 48.5 $\pm$ 10.4}
            & {\color{brown} 50.6 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 56.4 $\pm$ 9.6}
            & {\color{brown} 51.8 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 69.0 $\pm$ 13.7} \\
        & & 25 $\%$
            & {\color{brown} 30.8 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 16.5 $\pm$ 3.6}
            & {\color{brown} 58.8 $\pm$ 5.9 $\%$} $\vert$\ {\color{teal} 42.5 $\pm$ 10.6}
            & {\color{brown} 27.1 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 4.5 $\pm$ 1.6}
            & {\color{brown} 20.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 3.7 $\pm$ 0.9} \\

        \hline

        % hopper-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.4 $\pm$ 0.6
            & 100.0 $\%$ $\vert$\ 98.3 $\pm$ 7.9 
            & 100.0 $\%$ $\vert$\ 109.9 $\pm$ 0.9
            & 100.0 $\%$ $\vert$\ 111.0 $\pm$ 0.4 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 91.6 $\pm$ 2.5 $\%$} $\vert$\ {\color{teal} 106.8 $\pm$ 3.0}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 79.5 $\pm$ 11.7}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 110.3 $\pm$ 1.2}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 111.4 $\pm$ 0.4} \\
        Expert & Hopper & 75 $\%$
            & {\color{brown} 66.4 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 94.9 $\pm$ 15.7}
            & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 37.0 $\pm$ 10.1}
            & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 76.5 $\pm$ 22.4}
            & {\color{brown} 76.4 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 79.5 $\pm$ 27.0} \\
        & & 50 $\%$
            & {\color{brown} 41.5 $\pm$ 2.9 $\%$} $\vert$\ {\color{teal} 29.3 $\pm$ 5.0}
            & {\color{brown} 41.8 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 14.3 $\pm$ 7.4}
            & {\color{brown} 47.3 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 41.3 $\pm$ 7.9}
            & {\color{brown} 47.3 $\pm$ 7.6 $\%$} $\vert$\ {\color{teal} 23.3 $\pm$ 9.0} \\
        & & 25 $\%$
            & {\color{brown} 18.2 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 13.5 $\pm$ 2.8}
            & {\color{brown} 10.9 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 1.8 $\pm$ 0.7}
            & {\color{brown} 18.2 $\pm$ 6.4 $\%$} $\vert$\ {\color{teal} 20.5 $\pm$ 13.7}
            & {\color{brown} 7.3 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 1.9 $\pm$ 1.1} \\

        \hline

        %walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.3 $\pm$ 0.3
            & 100.0 $\%$ $\vert$\ 112.2 $\pm$ 2.1 
            & 100.0 $\%$ $\vert$\ 108.8 $\pm$ 0.3
            & 100.0 $\%$ $\vert$\ 108.9 $\pm$ 0.2 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 94.8 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 109.0 $\pm$ 0.5}
            & {\color{brown} 91.8 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 108.2 $\pm$ 2.7}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.9 $\pm$ 0.3}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 109.1 $\pm$ 0.2} \\
        Expert & Walker2D & 75 $\%$
            & {\color{brown} 66.5 $\pm$ 2.5 $\%$} $\vert$\ {\color{teal} 108.3 $\pm$ 1.1}
            & {\color{brown} 75.3 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 80.3 $\pm$ 16.8}
            & {\color{brown} 70.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 106.0 $\pm$ 1.6}
            & {\color{brown} 70.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 101.2 $\pm$ 8.7} \\
        & & 50 $\%$
            & {\color{brown} 46.2 $\pm$ 3.6 $\%$} $\vert$\ {\color{teal} 91.3 $\pm$ 6.2}
            & {\color{brown} 49.4 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 10.1 $\pm$ 3.4}
            & {\color{brown} 49.4 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 28.0 $\pm$ 13.2}
            & {\color{brown} 51.8 $\pm$ 4.9 $\%$} $\vert$\ {\color{teal} 10.0 $\pm$ 1.0} \\
        & & 25 $\%$
            & {\color{brown} 20.0 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 13.9 $\pm$ 1.2}
            & {\color{brown} 25.9 $\pm$ 5.3 $\%$} $\vert$\ {\color{teal} 6.1 $\pm$ 4.5}
            & {\color{brown} 25.9 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 8.9 $\pm$ 1.0}
            & {\color{brown} 25.9 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 3.9 $\pm$ 2.0} \\

        \hline
        \hline
        \SetCell[c=2]{c}{} & & baseline
            & 100.0 $\%$ $\vert$\ 103.7
            & 100.0 $\%$ $\vert$\ 100.6
            & 100.0 $\%$ $\vert$\ 103.7
            & 100.0 $\%$ $\vert$\ 104.0 \\
        \hline
        \SetCell[c=2]{c}{} & & 100 $\%$
            & {\color{brown} 95.2 $\%$} $\vert$\ {\color{teal} 103.1}
            & {\color{brown} 96.5 $\%$} $\vert$\ {\color{teal} 87.5}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 103.6}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 104.3} \\
        \SetCell[c=2]{c}{Average} & & 75 $\%$
            & {\color{brown} 65.5 $\%$} $\vert$\ {\color{teal} 96.1}
            & {\color{brown} 76.0 $\%$} $\vert$\ {\color{teal} 59.8}
            & {\color{brown} 71.3 $\%$} $\vert$\ {\color{teal} 90.3}
            & {\color{brown} 73.3 $\%$} $\vert$\ {\color{teal} 88.9} \\
        \SetCell[c=2]{c}{} & & 50 $\%$
            & {\color{brown} 44.3 $\%$} $\vert$\ {\color{teal} 71.3}
            & {\color{brown} 51.2 $\%$} $\vert$\ {\color{teal} 20.4}
            & {\color{brown} 48.3 $\%$} $\vert$\ {\color{teal} 38.6}
            & {\color{brown} 49.5 $\%$} $\vert$\ {\color{teal} 33.1} \\
        \SetCell[c=2]{c}{} & & 25 $\%$
            & {\color{brown} 24.2 $\%$} $\vert$\ {\color{teal} 14.8}
            & {\color{brown} 31.9 $\%$} $\vert$\ {\color{teal} 16.6}
            & {\color{brown} 22.9 $\%$} $\vert$\ {\color{teal} 10.7}
            & {\color{brown} 17.7 $\%$} $\vert$\ {\color{teal} 2.9} \\

        \hline
        
    \end{tblr}
    \caption{\textbf{\textcolor{blue}{NEW RESULTS}} {\color{brown}Average Cost} \& {\color{teal}Average Performance} on D4RL environments for the \textbf{Expert  datasets}.}    
   \label{new_budget_rewards_d4rl_xp}
\end{table*}

==> tables/new/budget_godot.tex <==
\begin{table*}[!h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-8} = {mygray},
        row{9} = {mydarkgray},
        row{16} = {mydarkgray},
        row{17-28} = {mygray},
        row{29} = {mydarkgray},
    }
        \hline
        \textbf{Environment} & \textbf{Type} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{RCBC}\\
        \hline
        
        % Easy-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 102.7 $\pm$ 0.8
            & 100.0 $\%$ $\vert$\ 101.1 $\pm$ 1.7 \\
        
        \hline
        
        & & & {\color{brown} 7.2 $\pm$ 1.5 $\%$} & {\color{brown} 0.0 $\pm$ 0.0 $\%$} \\
        EasyMap & Expert & 1 $\%$
        & {\color{teal}R = 97.2 $\pm$ 0.9} & {\color{teal}R = 87.9 $\pm$ 1.9} \\
        & & & {\color{teal}-} & {\color{teal}-} \\
        
        \hline
        
        & & & {\color{brown} 6.0 $\pm$ 2.9 $\%$} & {\color{brown} 0.0 $\pm$ 0.0 $\%$} \\
        EasyMap & Intermediate & 0 $\%$
        & {\color{teal}R = 91.9 $\pm$ 4.3} & {\color{teal}R = 88.2 $\pm$ 0.8} \\
        & & & {\color{teal}-} & {\color{teal}-} \\
        
        \hline
        
        % Easy-intermediate
        & & baseline
            & 100.0 $\%$ $\vert$\ 101.9 $\pm$ 1.0
            & 100.0 $\%$ $\vert$\ 102.5 $\pm$ 0.7 \\
        
        \hline
        
        & & & {\color{brown} 6.7 $\pm$ 4.9 $\%$} & {\color{brown} 0.0 $\pm$ 0.0 $\%$} \\
        EasyMap & Intermediate & 1 $\%$
        & {\color{teal}R = 98.7 $\pm$ 1.1} & {\color{teal}R = 93.1 $\pm$ 1.8} \\
        & & & {\color{teal}-} & {\color{teal}-} \\
        
        \hline
        
        & & & {\color{brown} 5.0 $\pm$ 3.0 $\%$} & {\color{brown} 0.0 $\pm$ 0.0 $\%$} \\
        EasyMap & Intermediate & 0 $\%$
        & {\color{teal}R = 96.6 $\pm$ 0.2} & {\color{teal}R = 92.0 $\pm$ 2.4} \\
        & & & {\color{teal}-} & {\color{teal}-} \\

        \hline

        % Hard-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 84.0 $\pm$ 0.5
            & 100.0 $\%$ $\vert$\ 72.4 $\pm$ 1.2 \\
        
        \hline
        
        & & & {\color{brown} 7.4 $\pm$ 0.5 $\%$} & {\color{brown} 6.4 $\pm$ 0.2 $\%$} \\
        Hard & Expert & 10 $\%$
        & {\color{teal}R = 47.4 $\pm$ 0.0} & {\color{teal}R = 53.6 $\pm$ 0.0} \\
        & & & {\color{teal}-} & {\color{teal}-} \\
        
        \hline
        
        & & & {\color{brown} 4.6 $\pm$ 0.5 $\%$} & {\color{brown} 2.8 $\pm$ 0.0 $\%$} \\
        Hard & Expert & 5 $\%$
        & {\color{teal}R = 44.2 $\pm$ 0.2} & {\color{teal}R = 46.8 $\pm$ 0.0} \\
        & & & {\color{teal}-} & {\color{teal}-} \\

        \hline
        
        & & & {\color{brown} 2.0 $\pm$ 0.1 $\%$} & {\color{brown} 1.2 $\pm$ 0.0 $\%$} \\
        Hard & Expert & 1 $\%$
        & {\color{teal}R = 43.0 $\pm$ 0.0} & {\color{teal}R = 41.0 $\pm$ 0.1} \\
        & & & {\color{teal}-} & {\color{teal}-} \\

        \hline
        
        & & & {\color{brown} 1.2 $\pm$ 0.1 $\%$} & {\color{brown} 0.2 $\pm$ 0.0 $\%$} \\
        Hard & Expert & 0 $\%$
        & {\color{teal}R = 35.4 $\pm$ 0.1} & {\color{teal}R = 25.1 $\pm$ 0.1} \\
        & & & {\color{teal}-} & {\color{teal}-} \\

        \hline

        % Hard-intermediate
        & & baseline
            & 100.0 $\%$ $\vert$\ 53.1 $\pm$ 4.3
            & 100.0 $\%$ $\vert$\ 49.0 $\pm$ 0.6 \\
        
        \hline
        
        & & & {\color{brown} 8.8 $\pm$ 0.1 $\%$} & {\color{brown} 8.1 $\pm$ 0.0 $\%$} \\
        Hard & Intermediate & 10 $\%$
        & {\color{teal}R = 44.2 $\pm$ 0.5} & {\color{teal}R = 49.1 $\pm$ 0.3} \\
        & & & {\color{teal}-} & {\color{teal}-} \\
        
        \hline
        
        & & & {\color{brown} 5.3 $\pm$ 0.2 $\%$} & {\color{brown} 4.4 $\pm$ 0.0 $\%$} \\
        Hard & Intermediate & 5 $\%$
        & {\color{teal}R = 39.2 $\pm$ 0.5} & {\color{teal}R = 45.7 $\pm$ 0.2} \\
        & & & {\color{teal}-} & {\color{teal}-} \\

        \hline
        
        & & & {\color{brown} 2.0 $\pm$ 0.0 $\%$} & {\color{brown} 3.1 $\pm$ 0.1 $\%$} \\
        Hard & Intermediate & 1 $\%$
        & {\color{teal}R = 39.2 $\pm$ 0.1} & {\color{teal}R = 41.0 $\pm$ 0.1} \\
        & & & {\color{teal}-} & {\color{teal}-} \\

        \hline
        
        & & & {\color{brown} 1.0 $\pm$ 0.1 $\%$} & {\color{brown} 2.7 $\pm$ 0.1 $\%$} \\
        Hard & Intermediate & 0 $\%$
        & {\color{teal}R = 31.8 $\pm$ 0.1} & {\color{teal}R = 42.1 $\pm$ 0.0} \\
        & & & {\color{teal}-} & {\color{teal}-} \\

        \hline
    
    \end{tblr}
    \caption{\textbf{\textcolor{red}{OLD RESULTS}} {\color{brown}Average Cost} \& {\color{teal}Average Performance} on the 3D environments.}    
   \label{old_budget_rewards_godot}
\end{table*}

\begin{table*}[!h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-14} = {mygray},
        row{15} = {mydarkgray},
        row{28} = {mydarkgray},
        row{29-40} = {mygray},
        row{41} = {mydarkgray},
    }
        \hline
        \textbf{Environment} & \textbf{Type} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % Easy-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 102.6 $\pm$ 0.6
            & 100.0 $\%$ $\vert$\ R = 101.9 $\pm$ 0.4
            & 100.0 $\%$ $\vert$\ R = 101.6 $\pm$ 0.4 \\
        
        \hline
        
        & & & {\color{brown} 12.5 $\pm$ 0.2 $\%$} & {\color{brown} 23.3 $\pm$ 0.3 $\%$} & {\color{brown} 19.2 $\pm$ 0.0 $\%$}\\
        EasyMap & Expert & 50 $\%$
        & {\color{teal}R = 102.3 $\pm$ 0.3} & {\color{teal}R = 101.8 $\pm$ 0.9} & {\color{teal}R = 101.6 $\pm$ 0.2}\\
        & & & {\color{teal}S = 96.2 $\pm$ 0.5} & {\color{teal}S = 95.8 $\pm$ 1.2} & {\color{teal}S = 95.0 $\pm$ 0.0}\\
        
        \hline
        
        & & & {\color{brown} 9.7 $\pm$ 0.2 $\%$} & {\color{brown} 8.0 $\pm$ 0.4 $\%$} & {\color{brown} 7.3 $\pm$ 1.0 $\%$}\\
        EasyMap & Expert & 10 $\%$
        & {\color{teal}R = 102.3 $\pm$ 0.4} & {\color{teal}R = 102.3 $\pm$ 0.3} & {\color{teal}R = 101.0 $\pm$ 1.0}\\
        & & & {\color{teal}S = 96.4 $\pm$ 0.4} & {\color{teal}S = 96.0 $\pm$ 0.5} & {\color{teal}S = 94.8 $\pm$ 1.6}\\
        
        \hline
        
        & & & {\color{brown} 4.2 $\pm$ 0.1 $\%$} & {\color{brown} 0.7 $\pm$ 0.2 $\%$} & {\color{brown} 0.9 $\pm$ 0.1 $\%$}\\
        EasyMap & Expert & 1 $\%$
        & {\color{teal}R = 101.6 $\pm$ 0.5} & {\color{teal}R = 102.1 $\pm$ 1.1} & {\color{teal}R = 101.3 $\pm$ 0.2}\\
        & & & {\color{teal}S = 95.3 $\pm$ 1.2} & {\color{teal}S = 96.7 $\pm$ 2.4} & {\color{teal}S = 95.2 $\pm$ 0.7}\\
        
        \hline
        
        & & & {\color{brown} 3.1 $\pm$ 0.4 $\%$} & {\color{brown} 0.1 $\pm$ 0.0 $\%$} & {\color{brown} 0.3 $\pm$ 0.2 $\%$}\\
        EasyMap & Expert & 0 $\%$
        & {\color{teal}R = 101.1 $\pm$ 0.0} & {\color{teal}R = 100.9 $\pm$ 1.7} & {\color{teal}R = 100.9 $\pm$ 0.6}\\
        & & & {\color{teal}S = 95.5 $\pm$ 0.7} & {\color{teal}S = 95.5 $\pm$ 0.7} & {\color{teal}S = 94.3 $\pm$ 0.5}\\

        \hline

        % Easy-intermediate
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 101.4 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ R = 101.9 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ R = 99.9 $\pm$ 1.0 \\
        
        \hline
        
        & & & {\color{brown} 15.4 $\pm$ 0.3 $\%$} & {\color{brown} 26.4 $\pm$ 0.5 $\%$} & {\color{brown} 21.4 $\pm$ 0.9 $\%$}\\
        EasyMap & Intermediate & 50 $\%$
        & {\color{teal}R = 99.2 $\pm$ 0.5} & {\color{teal}R = 101.3 $\pm$ 0.2} & {\color{teal}R = 99.7 $\pm$ 2.2}\\
        & & & {\color{teal}S = 94.0 $\pm$ 0.7} & {\color{teal}S = 95.5 $\pm$ 0.2} & {\color{teal}S = 93.7 $\pm$ 2.8}\\
        
        \hline
        
        & & & {\color{brown} 9.3 $\pm$ 0.2 $\%$} & {\color{brown} 7.8 $\pm$ 0.5 $\%$} & {\color{brown} 7.4 $\pm$ 0.6 $\%$}\\
        EasyMap & Intermediate & 10 $\%$
        & {\color{teal}R = 99.9 $\pm$ 0.1} & {\color{teal}R = 101.5 $\pm$ 0.2} & {\color{teal}R = 98.7 $\pm$ 0.6}\\
        & & & {\color{teal}S = 94.7 $\pm$ 0.1} & {\color{teal}S = 95.5 $\pm$ 0.2} & {\color{teal}S = 93.3 $\pm$ 0.9}\\
        
        \hline
        
        & & & {\color{brown} 2.6 $\pm$ 0.3 $\%$} & {\color{brown} 1.0 $\pm$ 0.0 $\%$} & {\color{brown} 1.2 $\pm$ 0.0 $\%$}\\
        EasyMap & Intermediate & 1 $\%$
        & {\color{teal}R = 99.4 $\pm$ 0.5} & {\color{teal}R = 99.0 $\pm$ 1.1} & {\color{teal}R = 99.4 $\pm$ 0.2}\\
        & & & {\color{teal}S = 94.5 $\pm$ 0.5} & {\color{teal}S = 93.8 $\pm$ 1.2} & {\color{teal}S = 93.3 $\pm$ 0.0}\\
        
        \hline
        
        & & & {\color{brown} 2.1 $\pm$ 0.4 $\%$} & {\color{brown} 0.4 $\pm$ 0.0 $\%$} & {\color{brown} 0.5 $\pm$ 0.1 $\%$}\\
        EasyMap & Intermediate & 0 $\%$
        & {\color{teal}R = 98.7 $\pm$ 0.0} & {\color{teal}R = 99.0 $\pm$ 1.7} & {\color{teal}R = 99.4 $\pm$ 0.6}\\
        & & & {\color{teal}S = 93.7 $\pm$ 0.0} & {\color{teal}S = 93.8 $\pm$ 1.6} & {\color{teal}S = 92.5 $\pm$ 0.7}\\

        \hline

        % Hard-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 82.7 $\pm$ 1.0
            & 100.0 $\%$ $\vert$\ R = 76.2 $\pm$ 1.0
            & 100.0 $\%$ $\vert$\ R = 77.6 $\pm$ 1.2 \\
        
        \hline
        
        & & & {\color{brown} 27.1 $\pm$ 1.1 $\%$} & {\color{brown} 36.4 $\pm$ 0.4 $\%$} & {\color{brown} 30.7 $\pm$ 0.4 $\%$}\\
        HardMap & Expert & 50 $\%$
        & {\color{teal}R = 82.4 $\pm$ 2.3} & {\color{teal}R = 74.9 $\pm$ 0.5} & {\color{teal}R = 72.1 $\pm$ 1.0}\\
        & & & {\color{teal}S = 80.0 $\pm$ 3.3} & {\color{teal}S = 70.0 $\pm$ 0.5} & {\color{teal}S = 66.8 $\pm$ 0.2}\\
        
        \hline
        
        & & & {\color{brown} 10.2 $\pm$ 0.1 $\%$} & {\color{brown} 7.7 $\pm$ 0.2 $\%$} & {\color{brown} 7.2 $\pm$ 0.2 $\%$}\\
        HardMap & Expert & 10 $\%$
        & {\color{teal}R = 78.8 $\pm$ 2.4} & {\color{teal}R = 72.5 $\pm$ 5.1} & {\color{teal}R = 70.1 $\pm$ 0.2}\\
        & & & {\color{teal}S = 77.3 $\pm$ 1.4} & {\color{teal}S = 68.3 $\pm$ 1.9} & {\color{teal}S = 65.3 $\pm$ 0.9}\\

        \hline
        
        & & & {\color{brown} 2.9 $\pm$ 0.0 $\%$} & {\color{brown} 0.8 $\pm$ 0.1 $\%$} & {\color{brown} 0.9 $\pm$ 0.2 $\%$}\\
        HardMap & Expert & 1 $\%$
        & {\color{teal}R = 71.6 $\pm$ 1.5} & {\color{teal}R = 53.0 $\pm$ 5.5} & {\color{teal}R = 56.7 $\pm$ 1.5}\\
        & & & {\color{teal}S = 70.2 $\pm$ 2.1} & {\color{teal}S = 53.5 $\pm$ 7.3} & {\color{teal}S = 54.3 $\pm$ 0.5}\\

        \hline
        
        & & & {\color{brown} 1.9 $\pm$ 0.0 $\%$} & {\color{brown} 0.3 $\pm$ 0.2 $\%$} & {\color{brown} 0.4 $\pm$ 0.0 $\%$}\\
        HardMap & Expert & 0 $\%$
        & {\color{teal}R = 68.7 $\pm$ 4.7} & {\color{teal}R = 46.9 $\pm$ 2.2} & {\color{teal}R = 45.0 $\pm$ 2.6}\\
        & & & {\color{teal}S = 69.3 $\pm$ 3.3} & {\color{teal}S = 46.5 $\pm$ 2.6} & {\color{teal}S = 44.2 $\pm$ 1.2}\\

        \hline

        % Hard-intermediate
        & & baseline
            & 100.0 $\%$ $\vert$\ R = 52.2 $\pm$ 1.7
            & 100.0 $\%$ $\vert$\ R = 50.2 $\pm$ 1.3
            & 100.0 $\%$ $\vert$\ R = 46.7 $\pm$ 1.4 \\
        
        \hline
        
        & & & {\color{brown} 27.1 $\pm$ 0.3 $\%$} & {\color{brown} 36.4 $\pm$ 0.2 $\%$} & {\color{brown} 30.7 $\pm$ 0.1 $\%$}\\
        HardMap & Intermediate & 50 $\%$
        & {\color{teal}R = 51.0 $\pm$ 0.5} & {\color{teal}R = 49.9 $\pm$ 1.3} & {\color{teal}R = 45.3 $\pm$ 0.5}\\
        & & & {\color{teal}S = 45.5 $\pm$ 0.7} & {\color{teal}S = 43.2 $\pm$ 0.2} & {\color{teal}S = 38.3 $\pm$ 0.9}\\
        
        \hline
        
        & & & {\color{brown} 9.6 $\pm$ 0.0 $\%$} & {\color{brown} 9.5 $\pm$ 0.7 $\%$} & {\color{brown} 8.8 $\pm$ 0.5 $\%$}\\
        HardMap & Intermediate & 10 $\%$
        & {\color{teal}R = 52.5 $\pm$ 0.9} & {\color{teal}R = 49.4 $\pm$ 1.2} & {\color{teal}R = 44.7 $\pm$ 0.8}\\
        & & & {\color{teal}S = 46.5 $\pm$ 0.2} & {\color{teal}S = 43.7 $\pm$ 2.8} & {\color{teal}S = 37.2 $\pm$ 0.7}\\

        \hline
        
        & & & {\color{brown} 1.9 $\pm$ 0.0 $\%$} & {\color{brown} 1.7 $\pm$ 0.0 $\%$} & {\color{brown} 1.6 $\pm$ 0.1 $\%$}\\
        HardMap & Intermediate & 1 $\%$
        & {\color{teal}R = 48.9 $\pm$ 0.4} & {\color{teal}R = 40.7 $\pm$ 0.5} & {\color{teal}R = 40.7 $\pm$ 1.4}\\
        & & & {\color{teal}S = 45.4 $\pm$ 2.3} & {\color{teal}S = 37.3 $\pm$ 0.5} & {\color{teal}S = 34.2 $\pm$ 0.7}\\

        \hline
        
        & & & {\color{brown} 1.2 $\pm$ 0.0 $\%$} & {\color{brown} 0.9 $\pm$ 0.0 $\%$} & {\color{brown} 1.2 $\pm$ 0.0 $\%$}\\
        HardMap & Intermediate & 0 $\%$
        & {\color{teal}R = 43.3 $\pm$ 3.0} & {\color{teal}R = 36.1 $\pm$ 0.3} & {\color{teal}R = 38.8 $\pm$ 0.2}\\
        & & & {\color{teal}S = 40.7 $\pm$ 2.8} & {\color{teal}S = 35.0 $\pm$ 0.9} & {\color{teal}S = 32.3 $\pm$ 0.5}\\

        \hline
    
    \end{tblr}
    \caption{\textbf{\textcolor{blue}{NEW RESULTS}} {\color{brown}Average Cost} \& {\color{teal}Average Performance} on the 3D environments.}    
   \label{newbudget_rewards_godot}
\end{table*}


==> tables/new/question_2_d4rl.tex <==
\begin{table*}[!h]    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {orange},
        row{2} = {mydarkgray},
        row{3-5} = {mygray},
        row{6} = {mydarkgray},
        row{10} = {mydarkgray},
        row{11-13} = {mygray},
        row{14} = {mydarkgray},
        row{18} = {mydarkgray},
        row{19-21} = {mygray},
        row{22} = {mydarkgray}
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{N = 1} & \textbf{N = 5} & \textbf{N = 10} \\
        \hline

        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 72.6 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 90.6 $\pm$ 0.9}
            & {\color{brown} 74.8 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 90.2 $\pm$ 0.3}
            & {\color{brown} 76.3 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 90.5 $\pm$ 0.2} \\
        Expert & HalfCheetah & 50 $\%$
            & {\color{brown} 47.2 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 81.0 $\pm$ 4.4}
            & {\color{brown} 49.8 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 84.8 $\pm$ 0.2}
            & {\color{brown} 51.6 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 88.3 $\pm$ 0.5} \\
        & & 25 $\%$
            & {\color{brown} 27.2 $\pm$ 3.0 $\%$} $\vert$\ {\color{teal} 44.7 $\pm$ 21.6}
            & {\color{brown} 28.5 $\pm$ 1.0 $\%$} $\vert$\ {\color{teal} 45.1 $\pm$ 19.5}
            & {\color{brown} 34.5 $\pm$ 3.3 $\%$} $\vert$\ {\color{teal} 45.3 $\pm$ 12.4} \\

        \hline

        % walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 72.2 $\pm$ 1.9 $\%$} $\vert$\ {\color{teal} 102.5 $\pm$ 5.9}
            & {\color{brown} 75.5 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 105.9 $\pm$ 4.9}
            & {\color{brown} 75.2 $\pm$ 3.3 $\%$} $\vert$\ {\color{teal} 108.2 $\pm$ 0.9} \\
        Expert & Walker2d & 50 $\%$
            & {\color{brown} 50.0 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 80.4 $\pm$ 0.5}
            & {\color{brown} 50.7 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 93.0 $\pm$ 1.8}
            & {\color{brown} 54.4 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 93.9 $\pm$ 1.7} \\
        & & 25 $\%$
            & {\color{brown} 26.5 $\pm$ 1.7 $\%$} $\vert$\ {\color{teal} 20.3 $\pm$ 6.2}
            & {\color{brown} 26.7 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 21.0 $\pm$ 4.7}
            & {\color{brown} 27.5 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 25.7 $\pm$ 10.2} \\
        
        \hline
        
        % halfcheetah-medium-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 69.9 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 83.2 $\pm$ 5.4}
            & {\color{brown} 73.0 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 86.3 $\pm$ 1.3}
            & {\color{brown} 73.4 $\pm$ 2.2 $\%$} $\vert$\ {\color{teal} 86.6 $\pm$ 4.0} \\
        Medium-Expert & HalfCheetah & 50 $\%$
            & {\color{brown} 45.1 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 83.2 $\pm$ 5.4}
            & {\color{brown} 47.7 $\pm$ 1.3 $\%$} $\vert$\ {\color{teal} 73.3 $\pm$ 5.5}
            & {\color{brown} 47.3 $\pm$ 2.4 $\%$} $\vert$\ {\color{teal} 62.7 $\pm$ 4.4} \\
        & & 25 $\%$
            & {\color{brown} 34.1 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 37.5 $\pm$ 2.5}
            & {\color{brown} 38.8 $\pm$ 3.5 $\%$} $\vert$\ {\color{teal} 41.3 $\pm$ 2.8}
            & {\color{brown} 42.8 $\pm$ 1.6 $\%$} $\vert$\ {\color{teal} 40.0 $\pm$ 3.4} \\

        \hline

        % walker2d-medium-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.1 $\pm$ 1.3
            & 100.0 $\%$ $\vert$\ 108.1 $\pm$ 1.3
            & 100.0 $\%$ $\vert$\ 108.1 $\pm$ 1.3 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 74.9 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 81.6 $\pm$ 14.0}
            & {\color{brown} 74.3 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 103.9 $\pm$ 4.3}
            & {\color{brown} 76.9 $\pm$ 1.9 $\%$} $\vert$\ {\color{teal} 92.6 $\pm$ 21.3} \\
        Medium-Expert & Walker2d & 50 $\%$
            & {\color{brown} 50.0 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 46.4 $\pm$ 32.4}
            & {\color{brown} 58.1 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 61.3 $\pm$ 6.4}
            & {\color{brown} 54.9 $\pm$ 1.9 $\%$} $\vert$\ {\color{teal} 75.0 $\pm$ 9.9} \\
        & & 25 $\%$
            & {\color{brown} 27.6 $\pm$ 6.5 $\%$} $\vert$\ {\color{teal} 5.3 $\pm$ 1.9}
            & {\color{brown} 23.4 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 16.6 $\pm$ 2.1}
            & {\color{brown} 33.1 $\pm$ 4.2 $\%$} $\vert$\ {\color{teal} 16.5 $\pm$ 16.4} \\
            
        \hline        
        
    \end{tblr}
    \caption{
    {\color{brown}Average Cost} \& {\color{teal}Average Performances} reached by Budgeted DT for different cost windows sizes $N$.}
    \label{a1_budget_rewards_d4rl_cost_window}
\end{table*}


==> tables/new/question_3_d4rl.tex <==
\begin{table*}[!h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|,
        row{1} = {magenta},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{11-14} = {mygray}
    }
        \hline
        \textbf{Cost Constraint} & \textbf{BDT using  only\\No Noisy} & \textbf{BDT using  only\\No Noisy + Low Noisy} & \textbf{BDT using  only\\No Noisy + Low Noisy + High Noisy}\\
        \hline
        baseline
            & 100.0 $\%$ $\vert$\ 92.5
            & 100.0 $\%$ $\vert$\ 92.5
            & 100.0 $\%$ $\vert$\ 92.5 \\
        \hline
        221.0
            & {\color{brown} 190.7 $\pm$ 6.7 $\%$} $\vert$\ {\color{teal} 73.5 $\pm$ 14.8}
            & {\color{brown} 180.0 $\pm$ 10.2 $\%$} $\vert$\ {\color{teal} 89.0 $\pm$ 2.1}
            & {\color{brown} 190.0 $\pm$ 5.7 $\%$} $\vert$\ {\color{teal} 91.0 $\pm$ 0.1} \\
            & N = 56.0 $\%$ $\vert$\ L = 0.0 $\%$ $\vert$\ H = 0.0 $\%$
            & N = 31.0 $\%$ $\vert$\ L = 88.8 $\%$ $\vert$\ H = 0.0 $\%$
            & N = 30.5 $\%$ $\vert$\ L = 90.0 $\%$ $\vert$\ H = 22.5 $\%$ \\
        \hline
        110.5
            & {\color{brown} 82.9 $\pm$ 8.6 $\%$} $\vert$\ {\color{teal} 22.0 $\pm$ 2.8}
            & {\color{brown} 88.6 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 88.5 $\pm$ 2.1}
            & {\color{brown} 97.9 $\pm$ 3.0 $\%$} $\vert$\ {\color{teal} 87.5 $\pm$ 0.7} \\
            & N = 24.5 $\%$ $\vert$\ L = 0.0 $\%$ $\vert$\ H = 0.0 $\%$
            & N = 5.0 $\%$ $\vert$\ L = 86.0 $\%$ $\vert$\ H = 0.0 $\%$
            & N = 5.5 $\%$ $\vert$\ L = 85.0 $\%$ $\vert$\ H = 42.5 $\%$ \\
        \hline
        22.1
            & {\color{brown} 8.8 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 4.5 $\pm$ 0.7}
            & {\color{brown} 29.6 $\pm$ 6.4 $\%$} $\vert$\ {\color{teal} 24.5 $\pm$ 17.7}
            & {\color{brown} 24.6 $\pm$ 0.9 $\%$} $\vert$\ {\color{teal} 20.0 $\pm$ 2.8} \\
            & N = 2.5 $\%$ $\vert$\ L = 0.0 $\%$ $\vert$\ H = 0.0 $\%$
            & N = 0.0 $\%$ $\vert$\ L = 34.5 $\%$ $\vert$\ H = 0.0 $\%$
            & N = 0.0 $\%$ $\vert$\ L = 24.5 $\%$ $\vert$\ H = 22.5 $\%$ \\
        \hline
    
    \end{tblr}
    \caption{{\color{brown}Average Cost} \& {\color{teal}Average Performances} reached by Budgeted DT on different noisy settings over the HalfCheetah environment using the Medium-Expert dataset. In this setup the features without any noise are worth 20, those with a low noise are worth 5 and the ones with a more important noise are worth 1. Since 17 features are originally available, the maximum cost constraint possible is $\mathbf{C}=17\times(20+5+1)=442$. We constraint our models to $50\%$, $25\%$ and $5\%$ of this value. We also provide the respective proportion of each features used (N, L, H) depending on their quality (not noisy, low noisy and high noisy).}
    \label{a1_budget_rewards_d4rl_noisy}

\end{table*}

==> tables/new/random.tex <==
\begin{table}[h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-4} = {mygray},
        row{5} = {mydarkgray},
        row{8} = {mydarkgray},
        row{9-10} = {mygray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{DT} & \textbf{DT RANDOM}\\
        \hline
            
        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1 \\
        \hline
        Expert & HalfCheetah & 50 $\%$
            & {\color{brown} 48.9 $\pm$ 1.4 $\%$} $\vert$\ {\color{teal} 69.5 $\pm$ 15.2}
            & {\color{brown} 48.8 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 4.3 $\pm$ 1.1} \\
        & & 25 $\%$
            & {\color{brown} 27.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 56.3 $\pm$ 0.0}
            & {\color{brown} 24.0 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 3.9 $\pm$ 0.9} \\

        \hline
            
        % hopper-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6 \\
        \hline
        Expert & Hopper & 50 $\%$
            & {\color{brown} 49.1 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 54.0 $\pm$ 11.5}
            & {\color{brown} 48.6 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 9.8 $\pm$ 10.8} \\
        & & 25 $\%$
            & {\color{brown} 29.0 $\pm$ 2.1 $\%$} $\vert$\ {\color{teal} 13.5 $\pm$ 3.2}
            & {\color{brown} 23.7 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 13.2 $\pm$ 3.3} \\

        \hline
            
        %walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.5 $\pm$ 0.8 \\
        \hline
        Expert & Walker2d & 50 $\%$
            & {\color{brown} 50.7 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 82.8 $\pm$ 13.4}
            & {\color{brown} 48.8 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 15.8 $\pm$ 1.1} \\
        & & 25 $\%$
            & {\color{brown} 27.0 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 21.8 $\pm$ 12.9}
            & {\color{brown} 24.0 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 5.8 $\pm$ 1.5} \\

        \hline
        
    \end{tblr}
    \caption{\textcolor{brown}{Average Cost} \& \textcolor{teal}{Average Performances} reached on D4RL datasets  ($N=1$) by BDT and BDT with features randomly sampled.}
    \label{table:random}
\end{table}


==> tables/new/random2.tex <==
\begin{table}[t]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-4} = {mygray},
        row{5} = {mydarkgray},
        row{8} = {mydarkgray},
        row{9-10} = {mygray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} &  \textbf{BDT RANDOM}\\
        \hline
            
        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1 \\
        \hline
        Expert & HalfCheetah & 50 $\%$
            & {\color{brown} 48.8 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 4.3 $\pm$ 1.1} \\
        & & 25 $\%$
            & {\color{brown} 24.0 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 3.9 $\pm$ 0.9} \\

        \hline
            
        % hopper-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6 \\
        \hline
        Expert & Hopper & 50 $\%$
            & {\color{brown} 48.6 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 9.8 $\pm$ 10.8} \\
        & & 25 $\%$
            & {\color{brown} 23.7 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 13.2 $\pm$ 3.3} \\

        \hline
            
        %walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.5 $\pm$ 0.8 \\
        \hline
        Expert & Walker2d & 50 $\%$
            & {\color{brown} 48.8 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 15.8 $\pm$ 1.1} \\
        & & 25 $\%$
            & {\color{brown} 24.0 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 5.8 $\pm$ 1.5} \\

        \hline
        
    \end{tblr}
    \caption{\textcolor{brown}{Average Cost} \& \textcolor{teal}{Average Performances} reached on D4RL datasets  ($N=1$) by BDT with features randomly sampled -- to compare with Figure \ref{fig:perf}.}
    \label{table:random}

\end{table}


==> tables/new/timegodot.tex <==
% \begin{table}[!t]
% \scriptsize
% \centering
% \begin{tabular}{|c{3cm}|c{3cm}|} 

%     \hline
    
%     Range of the ray cast (in meters) & Compute Time (micro-seconds)  \\
    
%     \hline
    
%     1   & 165.05 \\
%     5   & 273    \\ 
%     10  & 329.08 \\
%     15  & 336.96 \\
%     20  & 343.42 \\ 
%     25  & 351.66 \\ 
%     50  & 382.54 \\ 
%     100 & 505.92 \\
    
%     \hline

% \end{tabular}
% \caption{Real timing to compute 48 raycasts on the 3D Navigation using Godot on a standard computer depending on the range of the raycasts using the Godot engine.}
% \label{fig:timegodot}
% \vspace{-0.6cm}
% \end{table}


\begin{table}[!h]
\scriptsize
\centering
\begin{tabular}{|c|c|} 

    \hline
    Range of the ray cast (in meters) & Compute Time (micro-seconds)  \\
    \hline
    1   & 2.58 \\
    5   & 4.27 \\ 
    10  & 5.14 \\ 
    25  & 5.37 \\ 
    50  & 5.49 \\ 
    100 & 7.9  \\
    \hline

\end{tabular}
\caption{Real timing to compute 64 raycasts on the 3D Navigation using the Godot engine on a standard computer depending on the range of the raycasts.}
\label{fig:new_timegodot}
\vspace{-0.6cm}
\end{table}

==> tables/question_1_d4rl_1.tex <==
\begin{table*}[!h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{7} = {mydarkgray},
        row{12} = {mydarkgray},
        row{13-16} = {mygray},
        row{17-21} = {mydarkgray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.4 $\pm$ 0.5
            & 100.0 $\%$ $\vert$\ 91.4 $\pm$ 2.3 
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.2
            & 100.0 $\%$ $\vert$\ 93.0 $\pm$ 0.2 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 97.5 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 92.4 $\pm$ 0.5}
            & {\color{brown} 97.6 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 85.9 $\pm$ 6.9}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 92.3 $\pm$ 0.2}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 93.0 $\pm$ 0.2} \\
        Expert & HalfCheetah & 75 $\%$
            & {\color{brown} 64.8 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 89.1 $\pm$ 1.2}
            & {\color{brown} 80.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 74.2 $\pm$ 3.9}
            & {\color{brown} 70.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 89.1 $\pm$ 1.1}
            & {\color{brown} 75.3 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 90.1 $\pm$ 1.0} \\
        & & 50 $\%$
            & {\color{brown} 44.5 $\pm$ 1.4 $\%$} $\vert$\ {\color{teal} 72.8 $\pm$ 6.5}
            & {\color{brown} 63.5 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 48.5 $\pm$ 10.4}
            & {\color{brown} 50.6 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 56.4 $\pm$ 9.6}
            & {\color{brown} 51.8 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 69.0 $\pm$ 13.7} \\
        & & 25 $\%$
            & {\color{brown} 30.8 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 16.5 $\pm$ 3.6}
            & {\color{brown} 58.8 $\pm$ 5.9 $\%$} $\vert$\ {\color{teal} 42.5 $\pm$ 10.6}
            & {\color{brown} 27.1 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 4.5 $\pm$ 1.6}
            & {\color{brown} 20.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 3.7 $\pm$ 0.9} \\

        \hline

        % hopper-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.4 $\pm$ 0.6
            & 100.0 $\%$ $\vert$\ 98.3 $\pm$ 7.9 
            & 100.0 $\%$ $\vert$\ 109.9 $\pm$ 0.9
            & 100.0 $\%$ $\vert$\ 111.0 $\pm$ 0.4 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 91.6 $\pm$ 2.5 $\%$} $\vert$\ {\color{teal} 106.8 $\pm$ 3.0}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 79.5 $\pm$ 11.7}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 110.3 $\pm$ 1.2}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 111.4 $\pm$ 0.4} \\
        Expert & Hopper & 75 $\%$
            & {\color{brown} 66.4 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 94.9 $\pm$ 15.7}
            & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 37.0 $\pm$ 10.1}
            & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 76.5 $\pm$ 22.4}
            & {\color{brown} 76.4 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 79.5 $\pm$ 27.0} \\
        & & 50 $\%$
            & {\color{brown} 41.5 $\pm$ 2.9 $\%$} $\vert$\ {\color{teal} 29.3 $\pm$ 5.0}
            & {\color{brown} 41.8 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 14.3 $\pm$ 7.4}
            & {\color{brown} 47.3 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 41.3 $\pm$ 7.9}
            & {\color{brown} 47.3 $\pm$ 7.6 $\%$} $\vert$\ {\color{teal} 23.3 $\pm$ 9.0} \\
        & & 25 $\%$
            & {\color{brown} 18.2 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 13.5 $\pm$ 2.8}
            & {\color{brown} 10.9 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 1.8 $\pm$ 0.7}
            & {\color{brown} 18.2 $\pm$ 6.4 $\%$} $\vert$\ {\color{teal} 20.5 $\pm$ 13.7}
            & {\color{brown} 7.3 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 1.9 $\pm$ 1.1} \\

        \hline

        %walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.3 $\pm$ 0.3
            & 100.0 $\%$ $\vert$\ 112.2 $\pm$ 2.1 
            & 100.0 $\%$ $\vert$\ 108.8 $\pm$ 0.3
            & 100.0 $\%$ $\vert$\ 108.9 $\pm$ 0.2 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 94.8 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 109.0 $\pm$ 0.5}
            & {\color{brown} 91.8 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 108.2 $\pm$ 2.7}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.9 $\pm$ 0.3}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 109.1 $\pm$ 0.2} \\
        Expert & Walker2D & 75 $\%$
            & {\color{brown} 66.5 $\pm$ 2.5 $\%$} $\vert$\ {\color{teal} 108.3 $\pm$ 1.1}
            & {\color{brown} 75.3 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 80.3 $\pm$ 16.8}
            & {\color{brown} 70.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 106.0 $\pm$ 1.6}
            & {\color{brown} 70.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 101.2 $\pm$ 8.7} \\
        & & 50 $\%$
            & {\color{brown} 46.2 $\pm$ 3.6 $\%$} $\vert$\ {\color{teal} 91.3 $\pm$ 6.2}
            & {\color{brown} 49.4 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 10.1 $\pm$ 3.4}
            & {\color{brown} 49.4 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 28.0 $\pm$ 13.2}
            & {\color{brown} 51.8 $\pm$ 4.9 $\%$} $\vert$\ {\color{teal} 10.0 $\pm$ 1.0} \\
        & & 25 $\%$
            & {\color{brown} 20.0 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 13.9 $\pm$ 1.2}
            & {\color{brown} 25.9 $\pm$ 5.3 $\%$} $\vert$\ {\color{teal} 6.1 $\pm$ 4.5}
            & {\color{brown} 25.9 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 8.9 $\pm$ 1.0}
            & {\color{brown} 25.9 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 3.9 $\pm$ 2.0} \\

        \hline
        \hline
        \SetCell[c=2]{c}{} & & baseline
            & 100.0 $\%$ $\vert$\ 103.7
            & 100.0 $\%$ $\vert$\ 100.6
            & 100.0 $\%$ $\vert$\ 103.7
            & 100.0 $\%$ $\vert$\ 104.0 \\
        \hline
        \SetCell[c=2]{c}{} & & 100 $\%$
            & {\color{brown} 95.2 $\%$} $\vert$\ {\color{teal} 103.1}
            & {\color{brown} 96.5 $\%$} $\vert$\ {\color{teal} 87.5}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 103.6}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 104.3} \\
        \SetCell[c=2]{c}{Average} & & 75 $\%$
            & {\color{brown} 65.5 $\%$} $\vert$\ {\color{teal} 96.1}
            & {\color{brown} 76.0 $\%$} $\vert$\ {\color{teal} 59.8}
            & {\color{brown} 71.3 $\%$} $\vert$\ {\color{teal} 90.3}
            & {\color{brown} 73.3 $\%$} $\vert$\ {\color{teal} 88.9} \\
        \SetCell[c=2]{c}{} & & 50 $\%$
            & {\color{brown} 44.3 $\%$} $\vert$\ {\color{teal} 71.3}
            & {\color{brown} 51.2 $\%$} $\vert$\ {\color{teal} 20.4}
            & {\color{brown} 48.3 $\%$} $\vert$\ {\color{teal} 38.6}
            & {\color{brown} 49.5 $\%$} $\vert$\ {\color{teal} 33.1} \\
        \SetCell[c=2]{c}{} & & 25 $\%$
            & {\color{brown} 24.2 $\%$} $\vert$\ {\color{teal} 14.8}
            & {\color{brown} 31.9 $\%$} $\vert$\ {\color{teal} 16.6}
            & {\color{brown} 22.9 $\%$} $\vert$\ {\color{teal} 10.7}
            & {\color{brown} 17.7 $\%$} $\vert$\ {\color{teal} 2.9} \\

        \hline
        
    \end{tblr}
    \caption{{\color{brown}Average Cost} \& {\color{teal}Average Performance} on D4RL environments for the \textbf{Expert  datasets}.}  
   \label{a1_budget_rewards_d4rl_expert_stochastic}
\end{table*}

% \begin{table*}[!ht]
%     \scriptsize
%     \centering
%     \begin{tblr}{
%         colspec = |c|c|c|c|c|c|c|c|c|,
%         row{1} = {lime},
%         row{2} = {mydarkgray},
%         row{3-6} = {mygray},
%         row{7} = {mydarkgray},
%         row{12} = {mydarkgray},
%         row{13-16} = {mygray},
%     }
%         \hline
%         \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{DT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
%         \hline

%         % halfcheetah-expert
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1
%             & 100.0 $\%$ $\vert$\ 91.6 $\pm$ 1.2 
%             & 100.0 $\%$ $\vert$\ 92.1 $\pm$ 0.7
%             & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 95.3 $\pm$ 1.2 $\%$} $\vert$\ {\color{teal} 90.8 $\pm$ 2.2}
%             & {\color{brown} 96.1 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 89.2 $\pm$ 4.9}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 92.8 $\pm$ 0.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 93.3 $\pm$ 0.1} \\
%         Expert & HalfCheetah & 75 $\%$
%             & {\color{brown} 72.6 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 90.6 $\pm$ 0.9}
%             & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 84.0 $\pm$ 3.4}
%             & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 91.1 $\pm$ 0.9}
%             & {\color{brown} 78.4 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 92.1 $\pm$ 0.6} \\
%         & & 50 $\%$
%             & {\color{brown} 47.2 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 81.0 $\pm$ 4.4}
%             & {\color{brown} 64.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 72.0 $\pm$ 5.2}
%             & {\color{brown} 52.9 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 81.8 $\pm$ 6.1}
%             & {\color{brown} 51.0 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 84.9 $\pm$ 1.6} \\
%         & & 25 $\%$
%             & {\color{brown} 27.2 $\pm$ 3.0 $\%$} $\vert$\ {\color{teal} 44.7 $\pm$ 21.6}
%             & {\color{brown} 62.7 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 59.5 $\pm$ 3.2}
%             & {\color{brown} 31.4 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 13.0 $\pm$ 13.6}
%             & {\color{brown} 29.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 5.8 $\pm$ 1.8} \\

%         \hline

%         % hopper-expert
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6
%             & 100.0 $\%$ $\vert$\ 89.7 $\pm$ 5.7 
%             & 100.0 $\%$ $\vert$\ 100.1 $\pm$ 15.2
%             & 100.0 $\%$ $\vert$\ 110.9 $\pm$ 0.7 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 84.2 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 103.0 $\pm$ 5.5}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 73.6 $\pm$ 11.3}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 110.7 $\pm$ 0.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 111.4 $\pm$ 0.4} \\
%         Expert & Hopper & 75 $\%$
%             & {\color{brown} 71.3 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 105.9 $\pm$ 2.7}
%             & {\color{brown} 75.8 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 44.5 $\pm$ 6.5}
%             & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 107.5 $\pm$ 3.3}
%             & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 98.1 $\pm$ 6.8} \\
%         & & 50 $\%$
%             & {\color{brown} 46.5 $\pm$ 4.8 $\%$} $\vert$\ {\color{teal} 56.9 $\pm$ 41.6}
%             & {\color{brown} 51.5 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 11.7 $\pm$ 4.2}
%             & {\color{brown} 54.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 48.0 $\pm$ 13.6}
%             & {\color{brown} 42.4 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 24.8 $\pm$ 13.6} \\
%         & & 25 $\%$
%             & {\color{brown} 28.4 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 16.9 $\pm$ 0.8}
%             & {\color{brown} 18.2 $\pm$ 9.1 $\%$} $\vert$\ {\color{teal} 6.4 $\pm$ 1.9}
%             & {\color{brown} 21.2 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 14.8 $\pm$ 3.3}
%             & {\color{brown} 15.2 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 7.5 $\pm$ 4.8} \\

%         \hline

%         %walker2d-expert
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 108.5 $\pm$ 0.8
%             & 100.0 $\%$ $\vert$\ 110.5 $\pm$ 0.5
%             & 100.0 $\%$ $\vert$\ 108.7 $\pm$ 0.1
%             & 100.0 $\%$ $\vert$\ 108.8 $\pm$ 0.1 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 94.5 $\pm$ 1.3 $\%$} $\vert$\ {\color{teal} 109.2 $\pm$ 0.7}
%             & {\color{brown} 88.2 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 103.7 $\pm$ 6.7}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 109.0 $\pm$ 0.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.8 $\pm$ 0.3 } \\
%         Expert & Walker2D & 75 $\%$
%             & {\color{brown} 72.2 $\pm$ 1.9 $\%$} $\vert$\ {\color{teal} 80.2 $\pm$ 46.1}
%             & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 102.5 $\pm$ 5.9}
%             & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 107.8 $\pm$ 0.5}
%             & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.8 $\pm$ 0.3} \\
%         & & 50 $\%$
%             & {\color{brown} 50.0 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 80.4 $\pm$ 16.0}
%             & {\color{brown} 52.9 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 14.2 $\pm$ 4.0}
%             & {\color{brown} 54.9 $\pm$ 6.8 $\%$} $\vert$\ {\color{teal} 62.7 $\pm$ 13.4}
%             & {\color{brown} 52.9 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 51.0 $\pm$ 16.9} \\
%         & & 25 $\%$
%             & {\color{brown} 26.5 $\pm$ 1.7 $\%$} $\vert$\ {\color{teal} 20.3 $\pm$ 6.2}
%             & {\color{brown} 25.5 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 8.7 $\pm$ 2.2}
%             & {\color{brown} 23.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 9.1 $\pm$ 2.3}
%             & {\color{brown} 27.5 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 11.1 $\pm$ 5.6} \\

%         \hline
        
%     \end{tblr}
%     \caption{\textcolor{orange}{[Anthony][Last results (BDT Walker2D 75$\%$ and BDT Hopper 50$\%$ could be further trained)]}\\
%     {\color{brown}Average Cost} \& {\color{teal}Average Performance} on OpenAI Gym environments datasets for a Cost Window of $N=1$.\\
%     We consider \textbf{deterministic query components}, and the agent have been trained on the \textbf{Expert datasets}.}
%     \label{1_budget_rewards_d4rl_expert_deterministic}
% \end{table*}

==> tables/question_1_d4rl_2.tex <==
\begin{table*}[h!]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{7} = {mydarkgray},
        row{12} = {mydarkgray},
        row{13-16} = {mygray},
        row{17-21} = {mydarkgray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % halfcheetah-medium-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.4
            & 100.0 $\%$ $\vert$\ 85.0 $\pm$ 5.6 
            & 100.0 $\%$ $\vert$\ 89.9 $\pm$ 0.4
            & 100.0 $\%$ $\vert$\ 45.7 $\pm$ 1.3 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 94.3 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 91.6 $\pm$ 1.0}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 82.4 $\pm$ 7.7}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 90.0 $\pm$ 1.1}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 44.3 $\pm$ 0.6} \\
        Med-Exp & HalfCheetah & 75 $\%$
            & {\color{brown} 65.8 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 86.8 $\pm$ 2.2}
            & {\color{brown} 84.7 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 63.8 $\pm$ 7.7}
            & {\color{brown} 76.5 $\pm$ 4.2 $\%$} $\vert$\ {\color{teal} 58.2 $\pm$ 3.3}
            & {\color{brown} 80.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 42.7 $\pm$ 0.8} \\
        & & 50 $\%$
            & {\color{brown} 43.5 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 53.3 $\pm$ 4.9}
            & {\color{brown} 80.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 54.1 $\pm$ 5.4}
            & {\color{brown} 54.1 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 19.6 $\pm$ 4.2}
            & {\color{brown} 47.1 $\pm$ 5.9 $\%$} $\vert$\ {\color{teal} 32.2 $\pm$ 7.7} \\
        & & 25 $\%$
            & {\color{brown} 26.4 $\pm$ 1.2 $\%$} $\vert$\ {\color{teal} 14.3 $\pm$ 2.0}
            & {\color{brown} 74.1 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 52.2 $\pm$ 4.1}
            & {\color{brown} 23.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 3.2 $\pm$ 0.4}
            & {\color{brown} 29.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 6.0 $\pm$ 1.1} \\

        \hline

        % hopper-medium-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.2 $\pm$ 4.4
            & 100.0 $\%$ $\vert$\ 100.1 $\pm$ 11.5 
            & 100.0 $\%$ $\vert$\ 107.6 $\pm$ 1.6
            & 100.0 $\%$ $\vert$\ 61.9 $\pm$ 3.9 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 96.1 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 105.1 $\pm$ 7.5}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 61.8 $\pm$ 34.3}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 101.8 $\pm$ 6.5}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 64.2 $\pm$ 4.9} \\
        Med-Exp & Hopper & 75 $\%$
            & {\color{brown} 67.8 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 105.1 $\pm$ 4.9}
            & {\color{brown} 80.0 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 22.1 $\pm$ 12.0}
            & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 52.0 $\pm$ 10.5}
            & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 47.1 $\pm$ 8.7} \\
        & & 50 $\%$
            & {\color{brown} 40.8 $\pm$ 3.3 $\%$} $\vert$\ {\color{teal} 34.3 $\pm$ 27.4}
            & {\color{brown} 50.9 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 8.1 $\pm$ 5.2}
            & {\color{brown} 45.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 37.0 $\pm$ 3.5}
            & {\color{brown} 41.8 $\pm$ 13.8 $\%$} $\vert$\ {\color{teal} 17.7 $\pm$ 14.6} \\
        & & 25 $\%$
            & {\color{brown} 16.7 $\pm$ 0.9 $\%$} $\vert$\ {\color{teal} 11.8 $\pm$ 10.7}
            & {\color{brown} 20.0 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 2.1 $\pm$ 1.0}
            & {\color{brown} 18.2 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 16.0 $\pm$ 7.5}
            & {\color{brown} 16.4 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 3.4 $\pm$ 2.3} \\

        \hline

        %walker2d-medium-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.5 $\pm$ 0.4
            & 100.0 $\%$ $\vert$\ 108.6 $\pm$ 2.3 
            & 100.0 $\%$ $\vert$\ 107.6 $\pm$ 1.7
            & 100.0 $\%$ $\vert$\ 108.6 $\pm$ 0.4 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 95.4 $\pm$ 0.9 $\%$} $\vert$\ {\color{teal} 108.1 $\pm$ 0.8}
            & {\color{brown} 94.1 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal}  111.3 $\pm$ 1.5}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 104.7 $\pm$ 3.6}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 107.9 $\pm$ 0.9} \\
        Med-Exp & Walker2D & 75 $\%$
            & {\color{brown} 66.0 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 102.2 $\pm$ 8.5}
            & {\color{brown} 84.7 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 79.9 $\pm$ 26.8}
            & {\color{brown} 70.6 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 44.9 $\pm$ 10.0}
            & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 49.4 $\pm$ 17.2} \\
        & & 50 $\%$
            & {\color{brown} 45.1 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 27.6 $\pm$ 4.5}
            & {\color{brown} 63.5 $\pm$ 9.7 $\%$} $\vert$\ {\color{teal} 9.1 $\pm$ 6.6}
            & {\color{brown} 54.1 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 10.4 $\pm$ 1.1}
            & {\color{brown} 51.8 $\pm$ 4.9 $\%$} $\vert$\ {\color{teal} 10.3 $\pm$ 2.3} \\
        & & 25 $\%$
            & {\color{brown} 18.7 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 4.2 $\pm$ 3.6}
            & {\color{brown} 49.4 $\pm$ 5.3 $\%$} $\vert$\ {\color{teal} 6.2 $\pm$ 3.4}
            & {\color{brown} 23.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 9.0 $\pm$ 1.7}
            & {\color{brown} 21.2 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 0.6 $\pm$ 1.6} \\

        \hline
        \hline
        \SetCell[c=2]{c}{} & & baseline
            & 100.0 $\%$ $\vert$\ 103.1
            & 100.0 $\%$ $\vert$\ 97.9
            & 100.0 $\%$ $\vert$\ 101.7
            & 100.0 $\%$ $\vert$\ 72.1 \\
        \hline
        \SetCell[c=2]{c}{} & & 100 $\%$
            & {\color{brown} 94.9 $\%$} $\vert$\ {\color{teal} 100.6}
            & {\color{brown} 98.0 $\%$} $\vert$\ {\color{teal} 83.5}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 97.4}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 71.2} \\
        \SetCell[c=2]{c}{Average} & & 75 $\%$
            & {\color{brown} 66.6 $\%$} $\vert$\ {\color{teal} 97.2}
            & {\color{brown} 83.1 $\%$} $\vert$\ {\color{teal} 52.0}
            & {\color{brown} 72.9 $\%$} $\vert$\ {\color{teal} 49.7}
            & {\color{brown} 76.4 $\%$} $\vert$\ {\color{teal} 43.4} \\
        \SetCell[c=2]{c}{} & & 50 $\%$
            & {\color{brown} 43.7 $\%$} $\vert$\ {\color{teal} 37.5}
            & {\color{brown} 64.8 $\%$} $\vert$\ {\color{teal} 23.0}
            & {\color{brown} 51.2 $\%$} $\vert$\ {\color{teal} 21.2}
            & {\color{brown} 46.5 $\%$} $\vert$\ {\color{teal} 19.0} \\
        \SetCell[c=2]{c}{} & & 25 $\%$
            & {\color{brown} 21.8 $\%$} $\vert$\ {\color{teal} 9.9}
            & {\color{brown} 46.6 $\%$} $\vert$\ {\color{teal} 19.4}
            & {\color{brown} 21.7 $\%$} $\vert$\ {\color{teal} 8.8}
            & {\color{brown} 21.5 $\%$} $\vert$\ {\color{teal} 3.0} \\

        \hline
        
    \end{tblr}
    \caption{{\color{brown}Average Cost} \& {\color{teal}Average Performance} on D4RL environments for the \textbf{Medium-Expert  datasets}.}
\label{a1_budget_rewards_d4rl_medium_expert_stochastic}
\end{table*}


% \begin{table*}[ht]
%     \scriptsize
%     \centering
%     \begin{tblr}{
%         colspec = |m{1cm}|c|c|c|c|c|c|c|c|,
%         row{1} = {lime},
%         row{2} = {mydarkgray},
%         row{3-6} = {mygray},
%         row{7} = {mydarkgray},
%         row{12} = {mydarkgray},
%         row{13-16} = {mygray},
%     }
%         \hline
%         \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{DT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
%         \hline
        
%         % halfcheetah-medium-expert
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7
%             & 100.0 $\%$ $\vert$\ 87.9 $\pm$ 2.2 
%             & 100.0 $\%$ $\vert$\ 86.1 $\pm$ 3.1
%             & 100.0 $\%$ $\vert$\ 49.5 $\pm$ 4.0 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 94.5 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 90.5 $\pm$ 0.9}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 86.5 $\pm$ 1.9}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 91.0 $\pm$ 0.3}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 70.5 $\pm$ 4.4} \\
%         Med-Exp & HalfCheetah & 75 $\%$
%             & {\color{brown} 69.9 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 83.2 $\pm$ 5.4}
%             & {\color{brown} 86.3 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 70.9 $\pm$ 9.8}
%             & {\color{brown} 82.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 76.2 $\pm$ 4.2}
%             & {\color{brown} 82.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 53.7 $\pm$ 3.6} \\
%         & & 50 $\%$
%             & {\color{brown} 45.1 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 63.9 $\pm$ 8.8}
%             & {\color{brown} 82.4 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 64.2 $\pm$ 11.6}
%             & {\color{brown} 54.9 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 32.2 $\pm$ 3.6}
%             & {\color{brown} 54.9 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 41.8 $\pm$ 0.8} \\
%         & & 25 $\%$
%             & {\color{brown} 38.8 $\pm$ 7.1 $\%$} $\vert$\ {\color{teal} 28.7 $\pm$ 8.2}
%             & {\color{brown} 84.3 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 68.5 $\pm$ 11.9}
%             & {\color{brown} 33.3 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 6.2 $\pm$ 3.2}
%             & {\color{brown} 35.3 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 29.2 $\pm$ 0.4} \\

%         \hline

%         % hopper-medium-expert
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 110.4 $\pm$ 0.8
%             & 100.0 $\%$ $\vert$\ 100.9 $\pm$ 7.8 
%             & 100.0 $\%$ $\vert$\ 89.4 $\pm$ 10.0
%             & 100.0 $\%$ $\vert$\ 49.8 $\pm$ 6.1 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 89.6 $\pm$ 3.1 $\%$} $\vert$\ {\color{teal} 103.3 $\pm$ 6.9}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 53.0 $\pm$ 19.8}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 109.5 $\pm$ 1.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 54.3 $\pm$ 1.9} \\
%         Med-Exp & Hopper & 75 $\%$
%             & {\color{brown} 76.6 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 93.7 $\pm$ 18.4}
%             & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 24.1 $\pm$ 9.0}
%             & {\color{brown} 72.7 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 76.4 $\pm$ 22.7}
%             & {\color{brown} 75.8 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 49.9 $\pm$ 3.4} \\
%         & & 50 $\%$
%             & {\color{brown} 52.5 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 79.2 $\pm$ 17.4}
%             & {\color{brown} 54.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 9.3 $\pm$ 11.9}
%             & {\color{brown} 54.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 49.3 $\pm$ 6.1}
%             & {\color{brown} 54.5 $\pm$ 9.1 $\%$} $\vert$\ {\color{teal} 34.8 $\pm$ 16.2} \\
%         & & 25 $\%$
%             & {\color{brown} 25.3 $\pm$ 5.5 $\%$} $\vert$\ {\color{teal} 19.5 $\pm$ 12.0}
%             & {\color{brown} 21.2 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 2.5 $\pm$ 1.3}
%             & {\color{brown} 27.3 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 6.4 $\pm$ 1.6}
%             & {\color{brown} 15.2 $\pm$ 5.2 $\%$} $\vert$\ {\color{teal} 2.8 $\pm$ 0.2} \\

%         \hline

%         %walker2d-medium-expert
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 108.1 $\pm$ 1.3
%             & 100.0 $\%$ $\vert$\ 109.1 $\pm$ 2.8 
%             & 100.0 $\%$ $\vert$\ 95.1 $\pm$ 14.5
%             & 100.0 $\%$ $\vert$\ 106.8 $\pm$ 2.4 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 96.4 $\pm$ 1.2 $\%$} $\vert$\ {\color{teal} 106.9 $\pm$ 3.1}
%             & {\color{brown} 94.1 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 109.2 $\pm$ 1.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.5 $\pm$ 1.4}
%             & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 108.0 $\pm$ 0.3} \\
%         Med-Exp & Walker2D & 75 $\%$
%             & {\color{brown} 74.9 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 81.6 $\pm$ 14.0}
%             & {\color{brown} 80.4 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 38.1 $\pm$ 11.4}
%             & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 101.2 $\pm$ 9.3}
%             & {\color{brown} 76.5 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 95.9 $\pm$ 9.6} \\
%         & & 50 $\%$
%             & {\color{brown} 50.0 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 46.4 $\pm$ 32.4}
%             & {\color{brown} 62.7 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 17.3 $\pm$ 14.2}
%             & {\color{brown} 54.9 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 22.6 $\pm$ 22.4}
%             & {\color{brown} 54.9 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 28.0 $\pm$ 12.8} \\
%         & & 25 $\%$
%             & {\color{brown} 27.6 $\pm$ 6.5 $\%$} $\vert$\ {\color{teal} 5.3 $\pm$ 1.9}
%             & {\color{brown} 62.7 $\pm$ 9.0 $\%$} $\vert$\ {\color{teal} 23.4 $\pm$ 9.4}
%             & {\color{brown} 21.6 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 8.8 $\pm$ 1.3}
%             & {\color{brown} 31.4 $\pm$ 3.4 $\%$} $\vert$\ {\color{teal} 8.0 $\pm$ 4.5} \\
        
%         \hline
        
%     \end{tblr}
%     \caption{\textcolor{orange}{[Anthony][Last results (BDT Walker2D 50$\%$ could be further trained)]}\\
%     {\color{brown}Average Cost} \& {\color{teal}Average Performances} reached on OpenAI Gym environments for a Cost Window of $N=1$.\\
%     We consider \textbf{deterministic query components}, and the agents have been trained on the \textbf{Medium-Expert datasets}.}
%     \label{1_budget_rewards_d4rl_medium_expert_detrministic}
% \end{table*}


==> tables/question_1_d4rl_3.tex <==
\begin{table*}[h!]
    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-6} = {mygray},
        row{7} = {mydarkgray},
        row{12} = {mydarkgray},
        row{13-16} = {mygray},
        row{17-21} = {mydarkgray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{BDT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
        \hline

        % halfcheetah-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 42.5 $\pm$ 0.2
            & 100.0 $\%$ $\vert$\ 47.3 $\pm$ 0.3 
            & 100.0 $\%$ $\vert$\ 42.7 $\pm$ 0.2
            & 100.0 $\%$ $\vert$\ 42.6 $\pm$ 1.3 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 98.9 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 42.9 $\pm$ 0.1}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 47.1 $\pm$ 0.4}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.6 $\pm$ 0.2}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.7 $\pm$ 0.2} \\
        Medium & Halfcheetah & 75 $\%$
            & {\color{brown} 67.2 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 42.6 $\pm$ 0.1}
            & {\color{brown} 81.2 $\pm$ 2.6 $\%$} $\vert$\ {\color{teal} 47.4 $\pm$ 0.2}
            & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.7 $\pm$ 0.1}
            & {\color{brown} 76.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 42.5 $\pm$ 0.6} \\
        & & 50 $\%$
            & {\color{brown} 44.1 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 40.9 $\pm$ 0.6}
            & {\color{brown} 70.6 $\pm$ 7.2 $\%$} $\vert$\ {\color{teal} 47.7 $\pm$ 0.4}
            & {\color{brown} 55.3 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 40.8 $\pm$ 0.9}
            & {\color{brown} 56.3 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 41.6 $\pm$ 1.2} \\
        & & 25 $\%$
            & {\color{brown} 24.0 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 30.5 $\pm$ 1.9}
            & {\color{brown} 61.2 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 47.7 $\pm$ 0.2}
            & {\color{brown} 23.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 10.9 $\pm$ 0.9}
            & {\color{brown} 28.2 $\pm$ 4.9 $\%$} $\vert$\ {\color{teal} 16.9 $\pm$ 4.6} \\

        \hline

        % hopper-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 64.3 $\pm$ 4.2
            & 100.0 $\%$ $\vert$\ 77.6 $\pm$ 5.8 
            & 100.0 $\%$ $\vert$\ 66.1 $\pm$ 2.6
            & 100.0 $\%$ $\vert$\ 54.8 $\pm$ 1.4 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 92.6 $\pm$ 1.7 $\%$} $\vert$\ {\color{teal} 66.4 $\pm$ 1.6}
            & {\color{brown} 94.5 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 72.7 $\pm$ 6.0}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 69.5 $\pm$ 3.5}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 56.0 $\pm$ 0.6} \\
        Medium & Hopper & 75 $\%$
            & {\color{brown} 64.9 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 87.4 $\pm$ 1.5}
            & {\color{brown} 74.5 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 74.5 $\pm$ 14.9}
            & {\color{brown} 69.1 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 55.8 $\pm$ 10.6}
            & {\color{brown} 74.5 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 47.5 $\pm$ 2.5} \\
        & & 50 $\%$
            & {\color{brown} 37.5 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 29.1 $\pm$ 12.8}
            & {\color{brown} 52.7 $\pm$ 7.6 $\%$} $\vert$\ {\color{teal} 11.9 $\pm$ 7.7}
            & {\color{brown} 45.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 40.5 $\pm$ 9.7}
            & {\color{brown} 36.4 $\pm$ 9.1 $\%$} $\vert$\ {\color{teal} 8.4 $\pm$ 4.8} \\
        & & 25 $\%$
            & {\color{brown} 17.7 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 13.7 $\pm$ 2.8}
            & {\color{brown} 12.7 $\pm$ 5.0 $\%$} $\vert$\ {\color{teal} 5.2 $\pm$ 2.4}
            & {\color{brown} 18.2 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 8.3 $\pm$ 3.7}
            & {\color{brown} 16.4 $\pm$ 4.1 $\%$} $\vert$\ {\color{teal} 4.5 $\pm$ 2.4} \\

        \hline

        %walker2d-medium
        & & baseline
            & 100.0 $\%$ $\vert$\ 71.0 $\pm$ 3.1
            & 100.0 $\%$ $\vert$\ 76.5 $\pm$ 3.1 
            & 100.0 $\%$ $\vert$\ 75.2 $\pm$ 1.2
            & 100.0 $\%$ $\vert$\ 73.2 $\pm$ 0.9 \\
        \hline
        & & 100 $\%$
            & {\color{brown} 99.3 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 75.3 $\pm$ 1.3}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 77.8 $\pm$ 7.6}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 73.7 $\pm$ 2.0}
            & {\color{brown} 100.0 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 73.0 $\pm$ 1.4} \\
        Medium & Walker2D & 75 $\%$
            & {\color{brown} 67.3 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 72.7 $\pm$ 5.3}
            & {\color{brown} 80.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 62.7 $\pm$ 25.5}
            & {\color{brown} 74.1 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 71.6 $\pm$ 4.1}
            & {\color{brown} 76.5 $\pm$ 4.2 $\%$} $\vert$\ {\color{teal} 69.1 $\pm$ 4.6} \\
        & & 50 $\%$
            & {\color{brown} 46.0 $\pm$ 2.5 $\%$} $\vert$\ {\color{teal} 17.4 $\pm$ 5.7}
            & {\color{brown} 62.4 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 17.0 $\pm$ 4.4}
            & {\color{brown} 56.5 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 30.5 $\pm$ 15.5}
            & {\color{brown} 52.9 $\pm$ 4.2 $\%$} $\vert$\ {\color{teal} 14.6 $\pm$ 14.0} \\
        & & 25 $\%$
            & {\color{brown} 19.0 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 1.3 $\pm$ 0.4}
            & {\color{brown} 42.4 $\pm$ 4.9 $\%$} $\vert$\ {\color{teal} 6.4 $\pm$ 1.3}
            & {\color{brown} 20.0 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 6.6 $\pm$ 1.2}
            & {\color{brown} 21.2 $\pm$ 3.2 $\%$} $\vert$\ {\color{teal} 4.4 $\pm$ 3.0} \\

        \hline
        \hline
        \SetCell[c=2]{c}{} & & baseline
            & 100.0 $\%$ $\vert$\ 59.3
            & 100.0 $\%$ $\vert$\ 67.1
            & 100.0 $\%$ $\vert$\ 61.3
            & 100.0 $\%$ $\vert$\ 56.9 \\
        \hline
        \SetCell[c=2]{c}{} & & 100 $\%$
            & {\color{brown} 98.2 $\%$} $\vert$\ {\color{teal} 61.7}
            & {\color{brown} 98.2 $\%$} $\vert$\ {\color{teal} 64.5}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 61.5}
            & {\color{brown} 100.0 $\%$} $\vert$\ {\color{teal} 56.6} \\
        \SetCell[c=2]{c}{Average} & & 75 $\%$
            & {\color{brown} 66.9 $\%$} $\vert$\ {\color{teal} 69.3}
            & {\color{brown} 78.6 $\%$} $\vert$\ {\color{teal} 59.6}
            & {\color{brown} 73.2 $\%$} $\vert$\ {\color{teal} 55.7}
            & {\color{brown} 75.8 $\%$} $\vert$\ {\color{teal} 51.1} \\
        \SetCell[c=2]{c}{} & & 50 $\%$
            & {\color{brown} 43.9 $\%$} $\vert$\ {\color{teal} 27.7}
            & {\color{brown} 61.9 $\%$} $\vert$\ {\color{teal} 24.9}
            & {\color{brown} 52.4 $\%$} $\vert$\ {\color{teal} 34.2}
            & {\color{brown} 48.2 $\%$} $\vert$\ {\color{teal} 20.7} \\
        \SetCell[c=2]{c}{} & & 25 $\%$
            & {\color{brown} 20.5 $\%$} $\vert$\ {\color{teal} 14.7}
            & {\color{brown} 37.8 $\%$} $\vert$\ {\color{teal} 19.5}
            & {\color{brown} 20.6 $\%$} $\vert$\ {\color{teal} 8.2}
            & {\color{brown} 20.7 $\%$} $\vert$\ {\color{teal} 8.0} \\

        \hline
        
    \end{tblr}
    \caption{{\color{brown}Average Cost} \& {\color{teal}Average Performance} on D4RL environments for the \textbf{Medium  datasets}.}
\label{a1_budget_rewards_d4rl_medium_stochastic}
\end{table*}


% \begin{table*}[ht]
%     \scriptsize
%     \centering
%     \begin{tblr}{
%         colspec = |c|c|c|c|c|c|c|c|c|,
%         row{1} = {lime},
%         row{2} = {mydarkgray},
%         row{3-6} = {mygray},
%         row{7} = {mydarkgray},
%         row{12} = {mydarkgray},
%         row{13-16} = {mygray},
%     }
%         \hline
%         \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{DT} & \textbf{IQL} & \textbf{RCBC} & \textbf{BC}\\
%         \hline
        
%         % halfcheetah-medium
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 42.7 $\pm$ 0.2
%             & 100.0 $\%$ $\vert$\ 47.3 $\pm$ 0.2 
%             & 100.0 $\%$ $\vert$\ 42.7 $\pm$ 0.3
%             & 100.0 $\%$ $\vert$\ 42.3 $\pm$ 0.2 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 99.0 $\pm$ 0.4 \%} $\vert$\ {\color{teal} 42.7 $\pm$ 0.4}
%             & {\color{brown} 100.0 $\pm$ 0.0\%} $\vert$\ {\color{teal} 47.4 $\pm$ 0.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 42.8 $\pm$ 0.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 42.7 $\pm$ 0.1} \\
%         Medium & HalfCheetah & 75 $\%$
%             & {\color{brown} 71.7 $\pm$ 0.3 \%} $\vert$\ {\color{teal} 42.8 $\pm$ 0.0}
%             & {\color{brown} 82.4 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 47.5 $\pm$ 0.1}
%             & {\color{brown} 78.4 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 42.9 $\pm$ 0.4}
%             & {\color{brown} 80.4 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 42.8 $\pm$ 0.2} \\
%         & & 50 $\%$
%             & {\color{brown} 47.0 $\pm$ 0.3 \%} $\vert$\ {\color{teal} 40.6 $\pm$ 0.4}
%             & {\color{brown} 78.4 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 47.6 $\pm$ 0.1}
%             & {\color{brown} 58.8 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 42.5 $\pm$ 0.4}
%             & {\color{brown} 58.8 $\pm$ 5.9 \%} $\vert$\ {\color{teal} 42.4 $\pm$ 0.4} \\
%         & & 25 $\%$
%             & {\color{brown} 34.0 $\pm$ 1.5 \%} $\vert$\ {\color{teal} 34.0 $\pm$ 3.4}
%             & {\color{brown} 78.4 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 47.7 $\pm$ 0.2}
%             & {\color{brown} 33.3 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 39.7 $\pm$ 2.4}
%             & {\color{brown} 41.2 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 37.7 $\pm$ 5.0} \\

%         \hline

%         % hopper-medium
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 65.0 $\pm$ 4.7
%             & 100.0 $\%$ $\vert$\ 88.0 $\pm$ 12.4 
%             & 100.0 $\%$ $\vert$\ 63.4 $\pm$ 3.5
%             & 100.0 $\%$ $\vert$\ 54.5 $\pm$ 2.1 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 84.5 $\pm$ 2.9 \%} $\vert$\ {\color{teal} 62.6 $\pm$ 7.2}
%             & {\color{brown} 93.9 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 70.8 $\pm$ 5.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 66.2 $\pm$ 4.7}
%             & {\color{brown} 100.0 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 57.7 $\pm$ 0.7} \\
%         Medium & Hopper & 75 $\%$
%             & {\color{brown} 81.1 $\pm$ 0.7 \%} $\vert$\ {\color{teal} 66.2 $\pm$ 3.7}
%             & {\color{brown} 78.8 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 89.6 $\pm$ 8.0}
%             & {\color{brown} 72.7 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 55.8 $\pm$ 8.8}
%             & {\color{brown} 69.7 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 47.6 $\pm$ 3.4} \\
%          & & 50 $\%$
%             & {\color{brown} 70.2 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 75.6 $\pm$ 9.5}
%             & {\color{brown} 51.5 $\pm$ 13.9 \%} $\vert$\ {\color{teal} 18.7 $\pm$ 15.6}
%             & {\color{brown} 51.5 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 40.7 $\pm$ 13.3}
%             & {\color{brown} 51.5 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 29.1 $\pm$ 20.8} \\
%         & & 25 $\%$
%             & {\color{brown} 47.9 $\pm$ 1.8 \%} $\vert$\ {\color{teal} 92.8 $\pm$ 0.3}
%             & {\color{brown} 15.2 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 7.9 $\pm$ 0.7}
%             & {\color{brown} 27.3 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 6.2 $\pm$ 1.3}
%             & {\color{brown} 21.2 $\pm$ 5.2 \%} $\vert$\ {\color{teal} 4.8 $\pm$ 0.6} \\

%         \hline

%         % walker2d-medium
%         & & baseline
%             & 100.0 $\%$ $\vert$\ 74.1 $\pm$ 0.8
%             & 100.0 $\%$ $\vert$\ 78.0 $\pm$ 1.9 
%             & 100.0 $\%$ $\vert$\ 74.2 $\pm$ 1.4
%             & 100.0 $\%$ $\vert$\ 71.2 $\pm$ 2.0 \\
%         \hline
%         & & 100 $\%$
%             & {\color{brown} 98.8 $\pm$ 0.6 \%} $\vert$\ {\color{teal} 71.4 $\pm$ 0.2}
%             & {\color{brown} 100.0 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 75.2 $\pm$ 3.0}
%             & {\color{brown} 100.0 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 75.4 $\pm$ 0.5}
%             & {\color{brown} 100.0 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 71.5 $\pm$ 3.0} \\
%         Medium & Walker2D & 75 $\%$
%             & {\color{brown} 73.9 $\pm$ 0.3 \%} $\vert$\ {\color{teal} 73.2 $\pm$ 2.6}
%             & {\color{brown} 84.3 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 81.2 $\pm$ 2.9}
%             & {\color{brown} 76.5 $\pm$ 0.0 \%} $\vert$\ {\color{teal} 73.1 $\pm$ 3.0}
%             & {\color{brown} 74.5 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 67.2 $\pm$ 4.8} \\
%         & & 50 $\%$
%             & {\color{brown} 51.3 $\pm$ 1.0 \%} $\vert$\ {\color{teal} 54.3 $\pm$ 7.1}
%             & {\color{brown} 62.7 $\pm$ 9.0 \%} $\vert$\ {\color{teal} 18.6 $\pm$ 15.4}
%             & {\color{brown} 52.9 $\pm$ 5.9 \%} $\vert$\ {\color{teal} 46.9 $\pm$ 18.9}
%             & {\color{brown} 54.9 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 52.4 $\pm$ 10.2} \\
%         & & 25 $\%$
%             & {\color{brown} 25.7 $\pm$ 2.2 \%} $\vert$\ {\color{teal} 0.9 $\pm$ 0.4}
%             & {\color{brown} 58.8 $\pm$ 5.9 \%} $\vert$\ {\color{teal} 18.5 $\pm$ 9.2}
%             & {\color{brown} 31.4 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 14.5 $\pm$ 8.4}
%             & {\color{brown} 37.3 $\pm$ 3.4 \%} $\vert$\ {\color{teal} 12.9 $\pm$ 7.6} \\

%         \hline
        
%     \end{tblr}
%     \caption{\textcolor{orange}{[Anthony][Last results (Hopper need to be further trained to respect the cost constraint)]}\\
%     {\color{brown}Average Cost} \& {\color{teal}Average Performances} reached on OpenAI Gym environments for a Cost Window of $N=1$.\\
%     We consider \textbf{deterministic query components}, and the agents have been trained on the \textbf{Medium datasets}.}
%     \label{1_budget_rewards_d4rl_medium_deterministic}
% \end{table*}

==> tables/question_2_d4rl.tex <==
\begin{table*}[!h]    
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {orange},
        row{2} = {mydarkgray},
        row{3-5} = {mygray},
        row{6} = {mydarkgray},
        row{10} = {mydarkgray},
        row{11-13} = {mygray},
        row{14} = {mydarkgray},
        row{18} = {mydarkgray},
        row{19-21} = {mygray},
        row{22} = {mydarkgray}
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{N = 1} & \textbf{N = 5} & \textbf{N = 10} \\
        \hline

        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 72.6 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 90.6 $\pm$ 0.9}
            & {\color{brown} 74.8 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 90.2 $\pm$ 0.3}
            & {\color{brown} 76.3 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 90.5 $\pm$ 0.2} \\
        Expert & HalfCheetah & 50 $\%$
            & {\color{brown} 47.2 $\pm$ 0.7 $\%$} $\vert$\ {\color{teal} 81.0 $\pm$ 4.4}
            & {\color{brown} 49.8 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 84.8 $\pm$ 0.2}
            & {\color{brown} 51.6 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 88.3 $\pm$ 0.5} \\
        & & 25 $\%$
            & {\color{brown} 27.2 $\pm$ 3.0 $\%$} $\vert$\ {\color{teal} 44.7 $\pm$ 21.6}
            & {\color{brown} 28.5 $\pm$ 1.0 $\%$} $\vert$\ {\color{teal} 45.1 $\pm$ 19.5}
            & {\color{brown} 34.5 $\pm$ 3.3 $\%$} $\vert$\ {\color{teal} 45.3 $\pm$ 12.4} \\

        \hline

        % walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 72.2 $\pm$ 1.9 $\%$} $\vert$\ {\color{teal} 102.5 $\pm$ 5.9}
            & {\color{brown} 75.5 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 105.9 $\pm$ 4.9}
            & {\color{brown} 75.2 $\pm$ 3.3 $\%$} $\vert$\ {\color{teal} 108.2 $\pm$ 0.9} \\
        Expert & Walker2d & 50 $\%$
            & {\color{brown} 50.0 $\pm$ 0.5 $\%$} $\vert$\ {\color{teal} 80.4 $\pm$ 0.5}
            & {\color{brown} 50.7 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 93.0 $\pm$ 1.8}
            & {\color{brown} 54.4 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 93.9 $\pm$ 1.7} \\
        & & 25 $\%$
            & {\color{brown} 26.5 $\pm$ 1.7 $\%$} $\vert$\ {\color{teal} 20.3 $\pm$ 6.2}
            & {\color{brown} 26.7 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 21.0 $\pm$ 4.7}
            & {\color{brown} 27.5 $\pm$ 0.3 $\%$} $\vert$\ {\color{teal} 25.7 $\pm$ 10.2} \\
        
        \hline
        
        % halfcheetah-medium-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7
            & 100.0 $\%$ $\vert$\ 92.5 $\pm$ 0.7 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 69.9 $\pm$ 0.4 $\%$} $\vert$\ {\color{teal} 83.2 $\pm$ 5.4}
            & {\color{brown} 73.0 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 86.3 $\pm$ 1.3}
            & {\color{brown} 73.4 $\pm$ 2.2 $\%$} $\vert$\ {\color{teal} 86.6 $\pm$ 4.0} \\
        Medium-Expert & HalfCheetah & 50 $\%$
            & {\color{brown} 45.1 $\pm$ 0.2 $\%$} $\vert$\ {\color{teal} 83.2 $\pm$ 5.4}
            & {\color{brown} 47.7 $\pm$ 1.3 $\%$} $\vert$\ {\color{teal} 73.3 $\pm$ 5.5}
            & {\color{brown} 47.3 $\pm$ 2.4 $\%$} $\vert$\ {\color{teal} 62.7 $\pm$ 4.4} \\
        & & 25 $\%$
            & {\color{brown} 34.1 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 37.5 $\pm$ 2.5}
            & {\color{brown} 38.8 $\pm$ 3.5 $\%$} $\vert$\ {\color{teal} 41.3 $\pm$ 2.8}
            & {\color{brown} 42.8 $\pm$ 1.6 $\%$} $\vert$\ {\color{teal} 40.0 $\pm$ 3.4} \\

        \hline

        % walker2d-medium-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.1 $\pm$ 1.3
            & 100.0 $\%$ $\vert$\ 108.1 $\pm$ 1.3
            & 100.0 $\%$ $\vert$\ 108.1 $\pm$ 1.3 \\
        \hline
        & & 75 $\%$
            & {\color{brown} 74.9 $\pm$ 1.8 $\%$} $\vert$\ {\color{teal} 81.6 $\pm$ 14.0}
            & {\color{brown} 74.3 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 103.9 $\pm$ 4.3}
            & {\color{brown} 76.9 $\pm$ 1.9 $\%$} $\vert$\ {\color{teal} 92.6 $\pm$ 21.3} \\
        Medium-Expert & Walker2d & 50 $\%$
            & {\color{brown} 50.0 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 46.4 $\pm$ 32.4}
            & {\color{brown} 58.1 $\pm$ 0.6 $\%$} $\vert$\ {\color{teal} 61.3 $\pm$ 6.4}
            & {\color{brown} 54.9 $\pm$ 1.9 $\%$} $\vert$\ {\color{teal} 75.0 $\pm$ 9.9} \\
        & & 25 $\%$
            & {\color{brown} 27.6 $\pm$ 6.5 $\%$} $\vert$\ {\color{teal} 5.3 $\pm$ 1.9}
            & {\color{brown} 23.4 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 16.6 $\pm$ 2.1}
            & {\color{brown} 33.1 $\pm$ 4.2 $\%$} $\vert$\ {\color{teal} 16.5 $\pm$ 16.4} \\
            
        \hline        
        
    \end{tblr}
    \caption{
    {\color{brown}Average Cost} \& {\color{teal}Average Performances} reached by Budgeted DT for different cost windows sizes $N$.}
    \label{a1_budget_rewards_d4rl_cost_window}
\end{table*}


==> tables/random.tex <==
\begin{table}[h]
    \scriptsize
    \centering
    \begin{tblr}{
        colspec = |c|c|c|c|c|c|c|c|c|,
        row{1} = {lime},
        row{2} = {mydarkgray},
        row{3-4} = {mygray},
        row{5} = {mydarkgray},
        row{8} = {mydarkgray},
        row{9-10} = {mygray},
    }
        \hline
        \textbf{Type} & \textbf{Environment} & \textbf{Cost Constraint} & \textbf{DT} & \textbf{DT RANDOM}\\
        \hline
            
        % halfcheetah-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 92.7 $\pm$ 0.1 \\
        \hline
        Expert & HalfCheetah & 50 $\%$
            & {\color{brown} 48.9 $\pm$ 1.4 $\%$} $\vert$\ {\color{teal} 69.5 $\pm$ 15.2}
            & {\color{brown} 48.8 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 4.3 $\pm$ 1.1} \\
        & & 25 $\%$
            & {\color{brown} 27.5 $\pm$ 0.0 $\%$} $\vert$\ {\color{teal} 56.3 $\pm$ 0.0}
            & {\color{brown} 24.0 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 3.9 $\pm$ 0.9} \\

        \hline
            
        % hopper-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 110.1 $\pm$ 1.6 \\
        \hline
        Expert & Hopper & 50 $\%$
            & {\color{brown} 49.1 $\pm$ 0.8 $\%$} $\vert$\ {\color{teal} 54.0 $\pm$ 11.5}
            & {\color{brown} 48.6 $\pm$ 0.1 $\%$} $\vert$\ {\color{teal} 9.8 $\pm$ 10.8} \\
        & & 25 $\%$
            & {\color{brown} 29.0 $\pm$ 2.1 $\%$} $\vert$\ {\color{teal} 13.5 $\pm$ 3.2}
            & {\color{brown} 23.7 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 13.2 $\pm$ 3.3} \\

        \hline
            
        %walker2d-expert
        & & baseline
            & 100.0 $\%$ $\vert$\ 108.5 $\pm$ 0.8 \\
        \hline
        Expert & Walker2d & 50 $\%$
            & {\color{brown} 50.7 $\pm$ 1.1 $\%$} $\vert$\ {\color{teal} 82.8 $\pm$ 13.4}
            & {\color{brown} 48.8 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 15.8 $\pm$ 1.1} \\
        & & 25 $\%$
            & {\color{brown} 27.0 $\pm$ 1.5 $\%$} $\vert$\ {\color{teal} 21.8 $\pm$ 12.9}
            & {\color{brown} 24.0 $\pm$ 0.0 $\%$} \vert\ {\color{teal} 5.8 $\pm$ 1.5} \\

        \hline
        
    \end{tblr}
    \caption{\textcolor{brown}{Average Cost} \& \textcolor{teal}{Average Performances} reached on D4RL datasets  ($N=1$) by BDT and BDT with features randomly sampled.}
    \label{table:random}
\end{table}

